Model-based Lookahead Reinforcement Learning

Model-based Reinforcement Learning (MBRL) allows data-efficient learning which is required in real world applications such as robotics. However, despite the impressive data-efficiency, MBRL does not achieve the final performance of state-of-the-art Model-free Reinforcement Learning (MFRL) methods. We leverage the strengths of both realms and propose an approach that obtains high performance with a small amount of data. In particular, we combine MFRL and Model Predictive Control (MPC). While MFRL's strength in exploration allows us to train a better forward dynamics model for MPC, MPC improves the performance of the MFRL policy by sampling-based planning. The experimental results in standard continuous control benchmarks show that our approach can achieve MFRL`s level of performance while being as data-efficient as MBRL.

==> Model-based Lookahead Reinforcement Learning (NIPS2019) (3)/custom1.tex <==
% # Customization 1
%
% This file sets up the conditional variable "draftmode" and uses packages which can be configured later.
%
% ## Usage
%
% 1. Insert the following code before all other `\usepackage` in the main TEX file:
% ```latex
% \input{custom1.tex}
% ```
% 2. Insert the following code after all other `\usepackage` in the max TEX file:
% ```latex
% \booltrue{draftmode}
% \input{custom2.tex}
% ```
% 3. (Optional) Insert `\draftmodereminder` in `\title{}`, for example:
% ```latex
% \title{\draftmodereminder Playing Atari with Deep Reinforcement Learning}
% ```
% 4. (Optional) Insert the following code after `\bibliography` in the main TEX file:
% ```latex
% \input{appendix.tex}
% ```
%
% ## Preparing Submitting Version
%
% Simply comment the line `\booltrue{draftmode}` to turn off the features in draft mode.
%
% ## Draft Mode Features
%
% 1. Make title red to remind it is in draft mode
% 2. Make hyperlinks easy to be spotted
% 3. Show fixme annotations
%
% ## Choosing Packages
%
% There are many package choices for a single purpose. It's recommended to select the package by the following order of preferences:
% 1. Choose more recently maintained packages
% 2. Choose packages with no compatibility issues
% 3. Choose simpler packages suited for your needs
% Do not use more than one packages at the same time.
%
% The following packages are grouped by functionality and ordered by recommended preferences.
%
% ### Bibliography Management
%
% 1. (Use default bibtex)
% 2. cite
% 3. natbib
% 4. biblatex
%
% ### Pseudocode
%
% 1. algorithmic
% 2. algorithmicx
% 3. algorithm2e
%
% ### Subfigures
%
% 1. subcaption
% 2. subfig
%
% ### Table Appearance
%
% 1. (Use default tabular)
% 2. array
% 3. booktabs
%
% ### Table Width
%
% 1. (Use default tabular)
% 2. tabu
% 3. tabulary
% 4. tabularx
%
% ## Support
%
% The customization files are maintained by Shawn Chang. Contact me at https://elsa-lab.slack.com/messages/D6UDNMT98/ if you have any questions.

%%% Internal Use %%%

% ## Use color – Colour control for LATEX documents
%
% This package is used for decorating texts with colors.
%
% CTAN: https://ctan.org/pkg/color

\usepackage{color}

% ## Use etoolbox – e-TEX tools for LATEX
%
% This package is used for providing conditional variables for internal usage.
%
% CTAN: https://ctan.org/pkg/etoolbox

\usepackage{etoolbox}

% ## Declare Draft Mode Variable
%
% Reference: https://en.wikibooks.org/wiki/LaTeX/Plain_TeX

\newbool{draftmode}
\boolfalse{draftmode}

%%% Optional Customization %%%

% You can safely comment the following packages if not used.

% ## Use afterpage – Execute command after the next page break
%
% This package can be used to move floats to the next page.
%
% ### Usage
%
% Surround the float with `\afterpage{<float>}` to make it appear after the current page.
%
% ### Examples
%
% Move the figure one column (or one page) later after the current column:
% ```latex
% \afterpage{
%     \begin{figure}[t]
%         \centering
%         \fbox{
%             \rule{0pt}{50pt}
%             \rule{50pt}{0pt}
%         }
%         \caption{A figure.}
%         \label{fig:figure}
%     \end{figure}
% }
% ```
%
% CTAN: https://ctan.org/pkg/afterpage

\usepackage{afterpage}

% ## Use algorithm
%
% This package provides a floating environment for wrapping pseudocode.
%
% This package is not compatible with the "algorithm2e" package.
%
% ### Usage
%
% Use the environment `\begin{algorithm}[<pos>]` like `\begin{figure}[<pos>]`.
%
% ### Examples
%
% The following example reproduces the algorithm in the paper "Playing Atari with Deep Reinforcement Learning":
% ```latex
% \begin{algorithm*}[t]
%     \caption{Deep Q-learning with Experience Replay}
%     \label{alg:deepq}
%     \begin{algorithmic}
%         \STATE Initialize replay memory $\mathcal{D}$ to capacity $N$
%         \STATE Initialize action-value function $Q$ with random weights
%         \FOR{episode $=1,M$}
%             \STATE Initialize sequence $s_1=\{x_1\}$ and preprocessed sequenced $\phi_1=\phi(s_1)$
%             \FOR{$t=1,T$}
%                 \STATE With probability $\epsilon$ select a random action $a_t$
%                 \STATE otherwise select $a_t=\max_a Q^*(\phi(s_t),a;\theta)$
%                 \STATE Execute action $a_t$ in emulator and observe reward $r_t$ and image $x_{t+1}$
%                 \STATE Set $s_{t+1}=s_t,a_t,x_{t+1}$ and preprocess $\phi_{t+1}=\phi(s_{t+1})$
%                 \STATE Store transition $(\phi_t,a_t,r_t,\phi_{t+1})$ in $\mathcal{D}$
%                 \STATE Sample random minibatch of transitions $(\phi_j,a_j,r_j,\phi_{j+1})$ from $\mathcal{D}$
%                 \STATE Set $y_j=
%                     \begin{cases}
%                         r_j & \text{for terminal } \phi_{j+1} \\
%                         r_j+\gamma\max_{a'}Q(\phi_{j+1},a';\theta) & \text{for non-terminal } \phi_{j+1}
%                     \end{cases}$
%                 \STATE Peform a gradient descent step on $(y_j-Q(\phi_j,a_j;\theta))^2$ according to equation 3
%             \ENDFOR
%         \ENDFOR
%     \end{algorithmic}
% \end{algorithm*}
% ```
% Note: The above example requires the "algorithmic" package.
%
% CTAN: https://ctan.org/pkg/algorithms
% Reference: https://en.wikibooks.org/wiki/LaTeX/Algorithms

\usepackage{algorithm}

% ## Use amsmath – AMS mathematical facilities for LATEX
%
% This package provides miscellaneous enhancements for improving the information structure and printed output of documents containing mathematical formulas.
%
% CTAN: https://ctan.org/pkg/amsmath
% Reference: https://tex.stackexchange.com/a/32102

\usepackage{amsmath}

% ## Use amssymb
%
% This package internally loads "amsfonts", which provides extended set of fonts for use in mathematics.
%
% Reference: https://tex.stackexchange.com/a/32102
% See also: https://ctan.org/pkg/amsfonts

\usepackage{amssymb}

% ## Use amsthm – Typesetting theorems (AMS style)
%
% This package helps to define theorem-like structures.
%
% CTAN: https://ctan.org/pkg/amsthm
% Reference: https://tex.stackexchange.com/a/32102

\usepackage{amsthm}

% ## Use appendix – Extra control of appendices
%
% This package provides various ways of formatting the titles of appendices.
%
% ### Usage
%
% Write the appendix content inside the `appendices` environment:
% ```latex
% \begin{appendices}
% <Appendix Content>
% \end{appendices}
% ```
% You can customize the appendix environment:
% 1. Customize the appendix title (Default is "Appendices"):
%   ```latex
%   \renewcommand{\appendixpagename}{Supplementary Material}
%   ```
% 2. Add the appendix title with the command `\appendixpage`.
% 3. Change the section numbering format (Default is `\renewcommand{\thesection}{\Alph{section}}`):
%   ```latex
%   \renewcommand{\thesection}{S.\arabic{section}}
%   ```
%
% ### Examples
%
% To begin the appendix section, add the following at the end of document:
% ```latex
% \begin{appendices}
% \section{Appendix 1}
% Dummy text.
% \end{appendices}
% ```
%
% CTAN: https://ctan.org/pkg/appendix

% \usepackage{appendix}

% ## Use array – Extending the array and tabular environments
%
% This package improves the appearance of tables.
%
% ### Usage
%
% The first `\hline` should be replaced with `\firsthline` and the last `\hline` should be replaced with `\lasthline` to fix the aligning problem with texts if you switch from "tabular" to this package.
%
% ### Examples
%
% ```latex
% \begin{table}[t]
%     \centering
%     \begin{tabular}{llr}
%         \firsthline
%         \multicolumn{2}{c}{Item} \\
%         \cline{1-2}
%         Animal    & Description & Price (\$) \\
%         \hline
%         Gnat      & per gram    & 13.65      \\
%                   & each        & 0.01       \\
%         Gnu       & stuffed     & 92.50      \\
%         Emu       & stuffed     & 33.33      \\
%         Armadillo & frozen      & 8.99       \\
%         \lasthline
%     \end{tabular}
%     \caption{A table.}
%     \label{tab:table}
% \end{table}
% ```
%
% CTAN: https://ctan.org/pkg/array
% Reference: https://en.wikibooks.org/wiki/LaTeX/Tables

\usepackage{array}

% ## Use booktabs – Publication quality tables in LATEX
%
% This package improves the appearance of tables.
%
% ### Usage
%
% This package provides several commands to replace `\hline` (with `\toprule`, `\midrule` and `\bottomrule`) and `\cline` (with `\cmidrule`) in "tabular" package:
% 1. `\toprule[<wd>]`: Producing a thick top line
% 2. `\midrule[<wd>]`: Producing a light dividing line
% 3. `\bottomrule[<wd>]`: Producing a thick bottom line
% 4. `\cmidrule[<wd>]{a-b}`: Producing a subline to extend over only some columns
% `<wd>` is the thickness of the line, it is not recommended to specify it for each line. It is more recommended to change the lengths `\lightrulewidth` (for `\midrule`) and `\heavyrulewidth` (for `\toprule` and `\bottomrule`) globally. If you want more than one `\cmidrule`, add a `\morecmidrules` between two `\cmidrule`.
%
% ### Examples
%
% ```latex
% \begin{table}[t]
%     \centering
%     \begin{tabular}{llr}
%         \toprule
%         \multicolumn{2}{c}{Item} \\
%         \cmidrule{1-2}
%         Animal    & Description & Price (\$) \\
%         \midrule
%         Gnat      & per gram    & 13.65      \\
%                   & each        & 0.01       \\
%         Gnu       & stuffed     & 92.50      \\
%         Emu       & stuffed     & 33.33      \\
%         Armadillo & frozen      & 8.99       \\
%         \bottomrule
%     \end{tabular}
%     \caption{A table.}
%     \label{tab:table}
% \end{table}
% ```
%
% CTAN: https://ctan.org/pkg/booktabs
% Reference: https://en.wikibooks.org/wiki/LaTeX/Tables

\usepackage{booktabs}

% ## Use caption – Customising captions in floating environments
%
% This package is used for reducing vertical spacing after tables.
%
% CTAN: https://ctan.org/pkg/caption

\usepackage{caption}
\captionsetup{compatibility=false}

% ## Use enumitem – Control layout of itemize, enumerate, description
%
% This package is used for reducing vertical spacing between enumerate items.
%
% CTAN: https://ctan.org/pkg/enumitem

\usepackage{enumitem}

% ## Use FiXme - Collaborative annotation tool for LATEX
%
% This package allows you to annotate the document.
%
% ### Usage
%
% You can use the following commands to add inline annotations:
% ```latex
% \fxnote{<note>}
% \fxwarning{<note>}
% \fxerror{<note>}
% \fxfatal{<note>}
%
% \fxnote*{<note>}{<text>}
% \fxwarning*{<note>}{<text>}
% \fxerror*{<note>}{<text>}
% \fxfatal*{<note>}{<text>}
% ```
%
% ### Examples
%
% Add the following line in the document:
% ```latex
% \fxwarning{should add reference here}
% \fxerror{the reference is wrong}
% \fxnote*{move to section 2}{We present the ﬁrst deep learning model...}
% \fxerror*{please add figure}{Figure ? provides sample screenshots...}
% ```
%
% CTAN: https://ctan.org/pkg/fixme

\usepackage{fixme}

% ## Use geometry – Flexible and complete interface to document dimensions
%
% This package is used to adjust page layout.
%
% ### Usage
%
% Use the command `\geometry{<options>}`. Available options are:
% 1. `hscale=<float>`: Set ratio of width of total body to paper width (Default: `0.7`)
% 2. `vscale=<float>`: Set ratio of height of total body to paper height (Default: `0.7`)
% 3. `footskip=<length>`: Set spacing between baseline of last line of text and baseline of footer
% 4. `footnotesep=<length>`: Set spacing between the bottom of text body and the top of footnote text
%
% ### Examples
%
% To make text more occupied on a page, write:
% ```latex
% \geometry{
%     hscale=0.75,
%     vscale=0.75
% }
% ```
%
% CTAN: https://ctan.org/pkg/geometry

% \usepackage{geometry}

% ## Use graphicx – Enhanced support for graphics
%
% This package allows you to import external graphics.
%
% ### Usage
%
% Insert the graphic with the command:
% ```latex
% \includegraphics[<options>]{<file>}
% ```
% The most common used option is `width=<value>`, which scales the graphic to this value.
%
% ### Examples
%
% To insert an image `image.png`, add:
% ```latex
% \includegraphics[width=.3\linewidth]{image.png}
% ```
% `width=.3\linewidth` scales the graphic down to 0.3 relative to the width of a line. Scaling down is usually used in subfigures.
%
% CTAN: https://ctan.org/pkg/graphicx
% Reference: https://en.wikibooks.org/wiki/LaTeX/Importing_Graphics

\usepackage{graphicx}

% ## Use mathtools – Mathematical tools to use with amsmath
%
% This package extends the functions in "amsmath" and provides formatting options to clean up common typesetting problems.
%
% ### Usage
%
% This package provides the following commands:
% 1. Removing horizontal spacing:
%   1. `\mathclap{<math>}`: Remove horizontal spacing in subscripts, superscripts and exponents
%   2. `\mathllap{<math>}`: Same as `\mathclap` but condense only the left side
%   3. `\mathrlap{<math>}`: Same as `\mathclap` but condense only the left side
% 2. Cramped style:
%   1. `\cramped{<math>}`: Bring the component down a little, useful with more than one level of exponents
%   2. `\crampedllap{<math>}`: Apply both `\mathllap` and `\cramped`
%   3. `\crampedrlap{<math>}`: Apply both `\mathrlap` and `\cramped`
%   4. `\crampedclap{<math>}`: Apply both `\mathclap` and `\cramped`
% 3. Smash operator: `\smashoperator[<pos>]{<operator-with-limits>}`: Ignore the sub- and superscript of an operator with limits, same as `\crampedclap` but you don't have to type `\crampedclap` for both sub- and superscript. Available `<pos>` options are:
%     1. `l`: Condense only the left side
%     2. `r`: Condense only the right side
%     3. `lr`: Condense both sides (Default)
% 4. Adjust limits: `\adjustlimits{<operator1>}_{<limit1>} {<operator2>}_{<limit2>}`: Make subscripts of complex limits align vertically
% 5. Reduce vertical space in alignment environment: `\SwapAboveDisplaySkip`: Reduce vertical space above an equation in alignment environment
% 6. Arrow-like symbols:
%   1. `\xleftrightarrow[<sub>]{<sup>}`: Left and right arrows on a single line
%   2. `\xRightarrow[<sub>]{<sup>}`: Right arrow on double lines
%   3. `\xLeftarrow[<sub>]{<sup>}`: Left arrow on double lines
%   4. `\xLeftrightarrow[<sub>]{<sup>}`: Left and right arrows on double lines
%   5. `\xrightharpoonup[<sub>]{<sup>}`: Right harpoon on a single line
%   6. `\xleftharpoonup[<sub>]{<sup>}`: Left harpoon on a single line
%   7. `\xrightleftharpoons[<sub>]{<sub>}`: Right harpoon on the top and left harpoon on the bottom, to form double lines
%   8. `\xleftrightharpoons[<sub>]{<sub>}`: Left harpoon on the top and right harpoon on the bottom, to form double lines
% 7. Brackets:
%   1. `\underbracket{<arg>}`: Put a square bracket under an equation
%   2. `\overbracket{<arg>}`: Put a square bracket over an equation
% 8. Braces:
%   1. `\underbrace{<arg>}`: Put a brace under an equation
%   2. `\overbrace{<arg>}`: Put a brace over an equation
% 9. Matrix environments:
%   1. `\begin{<type>matrix*}[<col>]`: Enhanced environment of `matrix`, `pmatrix`, `bmatrix`, `Bmatrix`, `vmatrix` and `Vmatrix`
%   2. `\begin{<type>smallmatrix*}[<col>]`: Small version of `matrix`, `pmatrix`, `bmatrix`, `Bmatrix`, `vmatrix` and `Vmatrix`
%   `<col>` is column alignment. Available options are:
%     1. `l`: Left-aligned columns
%     2. `r`: Right-aligned columns
%     3. `c`: Center-aligned columns (Default)
% 10. Cases-like environments:
%   Similar to `cases` environment but set the rows in display style.
%   1. `\begin{dcases}`: Case with left brace
%   2. `\begin{rcases}`: Case with right brace
%   3. `\begin{drcases}`: Case with both left and right braces
%   Add a `*` after the above environment names to set the second column in normal Roman font.
% 11. Move equation left: `\MoveEqLeft[<number>]`: Move the long equation in alignment environment left by `<number>` ems if the line is unable to be aligned properly (Default `<number>`: 2)
% 12. Arrows between lines:
%   1. `\ArrowBetweenLines[<symbol>]`: Add symbol between two lines on the left
%   2. `\ArrowBetweenLines*[<symbol>]`: Add symbol between two lines on the right
%   (Default `<symbol>`: `\Updownarrow`)
% 13. Centered vertical dots:
%   1. `\vdotswithin{<symbol>}`: Vertical dots centered with symbol `<symbol>` in alignment environment
%   2. `\shortvdotswithin{<symbol>}`: Same as `\vdotswithin` but with reduced vertical margin
% 14. Short intertext: `\shortintertext{<text>}`: Same as `\intertext` provided by "amsmath" package but with reduced vertical spacing
% 15. Split fractions:
%   1. `\splitfrac{<numer>}{<denom>}`: Split long numerator or denominator into multilines
%   2. `\splitfrac{<numer>}{<denom>}`: Same as `\splitfrac` but with larger vertical spacing
%
% ### Examples
%
% ```latex
% % 1. Removing horizontal spacing
% \begin{equation}
%     A = \sum_{\mathclap{1\le i\le j\le n}} X_{ij},
%     B = \sum_{1\le i\le j\le n} X_{ij}
%     \label{eq:equation1}
% \end{equation}
% % 2. Cramped style
% \begin{equation}
%     A = \cramped{x^{x^2}},
%     B = x^{x^2}
%     \label{eq:equation2}
% \end{equation}
% % 3. Smash operator
% \begin{equation}
%     A = \smashoperator{\sum_{1\le i\le j\le n}^{3456}} X_{ij},
%     B = \sum_{1\le i\le j\le n}^{3456}
%     \label{eq:equation3}
% \end{equation}
% % 4. Adjust limits
% \begin{equation}
%     A = \adjustlimits\lim_{n\to\infty} \max_{p^2\ge K},
%     B = \lim_{n\to\infty} \max_{p^2\ge K}
%     \label{eq:equation4}
% \end{equation}
% % 6. Arrow-like symbols (1)
% \begin{equation}
%     A = x \xleftrightarrow[under]{over} y,
%     B = x \underset{under}{\overset{over}{\longleftrightarrow}} y
%     \label{eq:equation5}
% \end{equation}
% % 6. Arrow-like symbols (2)
% \begin{equation}
%     A = x \xrightharpoonup[under]{over} y,
%     B = x \underset{under}{\overset{over}{\rightharpoonup}} y
%     \label{eq:equation6}
% \end{equation}
% % 7. Brackets
% \begin{equation}
%     A = \underbracket{foo\ bar}_{under} = \overbracket{foo\ bar}^{over}
%     \label{eq:equation7}
% \end{equation}
% % 8. Braces
% \begin{equation}
%     A = \underbrace{foo\ bar}_{under} = \overbrace{foo\ bar}^{over},
%     B = \LaTeXunderbrace{foo\ bar}_{under} = \LaTeXoverbrace{foo\ bar}^{over}
%     \label{eq:equation8}
% \end{equation}
% % 9. Matrix environments (1)
% \begin{equation}
%     A = \begin{pmatrix*}[r]
%             -1 & 3 \\
%             2 & -4 \\
%         \end{pmatrix*},
%     B = \begin{pmatrix}
%             -1 & 3 \\
%             2 & -4 \\
%         \end{pmatrix}
%     \label{eq:equation9}
% \end{equation}
% % 9. Matrix environments (2)
% \begin{equation}
%     A = \begin{vsmallmatrix*}[r]
%             -1 & 3 \\
%             2 & -4 \\
%         \end{vsmallmatrix*},
%     B = \lvert
%         \begin{smallmatrix}
%             -1 & 3 \\
%             2 & -4 \\
%         \end{smallmatrix}\rvert
%     \label{eq:equation10}
% \end{equation}
% % 10. Cases-like environments
% \begin{equation}
%     \begin{alignedat}{2}
%         % 5. Reduce vertical space in alignment environment
%         \SwapAboveDisplaySkip
%         A &= \begin{dcases}
%                 E = m c^2 & c \approx 3.00\times 10^{8}\,\mathrm{m}/\mathrm{s} \\
%                 \int x-3\, dx & \text{Integral is display style} \\
%             \end{dcases} \\
%         B &= \begin{cases}
%                 E = m c^2 & c \approx 3.00\times 10^{8}\,\mathrm{m}/\mathrm{s} \\
%                 \int x-3\, dx & \text{Integral is display style} \\
%             \end{cases} \\
%     \end{alignedat}
%     \label{eq:equation11}
% \end{equation}
% % 11. Move equation left
% \begin{equation}
%     \begin{alignedat}{1}
%         \MoveEqLeft \text{A is really long text} \\
%         & = \dots \\
%         & \leq \dots \\
%         \text{B is really long text} \\
%         & = \dots \\
%         & \leq \dots \\
%     \end{alignedat}
%     \label{eq:equation12}
% \end{equation}
% % 12. Arrows between lines
% \begin{equation}
%     \begin{alignedat}{2}
%         a_1 &= 1 \\
%         \ArrowBetweenLines[\Downarrow]
%         a_2 &= a_1 + x \\
%         \ArrowBetweenLines*[\uparrow]
%         a_3 &= a_2 + x^2 \\
%     \end{alignedat}
%     \label{eq:equation13}
% \end{equation}
% % 13. Centered vertical dots
% \begin{equation}
%     \begin{alignedat}{2}
%         a_1 &= 1 \\
%         & \vdotswithin{=} \\
%         a_2 &= a_1 + x \\
%         \shortvdotswithin{=}
%         a_3 &= a_2 + x^2 \\
%     \end{alignedat}
%     \label{eq:equation14}
% \end{equation}
% % 14. Short intertext
% \begin{align}
%     a_1 &= 1 \shortintertext{A (\texttt{\small\textbackslash shortintertext})} \label{eq:equation15}
%     a_2 &= a_1 + x \intertext{B (\texttt{\small\textbackslash intertext})} \label{eq:equation16}
%     a_3 &= a_2 + x^2 \\ \label{eq:equation17}
% \end{align}
% % 15. Split fractions
% \begin{equation}
%     A = \frac{\splitfrac{xy + xy + xy + xy + xy}{+ xy + xy + xy + xy}}{z}
%     \label{eq:equation18}
% \end{equation}
% ```
%
% CTAN: https://ctan.org/pkg/mathtools
% Reference: https://www.overleaf.com/learn/latex/Articles/Mathtools_-_for_beautiful_math

\usepackage{mathtools}

% ## Use microtype – Subliminal refinements towards typographical perfection
%
% This package greatly improves general appearance of the text.
%
% Using this package will make a single line more likely to contain more words, thus reducing the overall space a paragraph occupies.
%
% CTAN: https://ctan.org/pkg/microtype
% Reference: http://www.khirevich.com/latex/microtype/

\usepackage{microtype}

% ## Use multirow – Create tabular cells spanning multiple rows
%
% This package is used for creating texts spanning multiple rows.
%
% ### Usage
%
% To create texts spanning multiple rows, use the command:
% ```latex
% \multirow[<vpos>]{<nrows>}{<width>}[<vmove>]{<text>}
% ```
% Available options are:
% 1. `<vpos>`: Vertical positioning of text
%   1. `c`: Vertically centered text (default)
%   2. 't': Top-aligned text
%   3. `b`: Bottom-aligned text
% 2. `<nrows>`: Number of rows to span
% 3. `<width>: Text width to be set
%   1. `*`: Use text parameter's natural width
%   2. `=`: Use specified width of column set by `\multirow`
% 4. `<vmove>`: The height of text to be raised. Use positive value to raise the text, or negative value to lower the text
% 5. `<text>`: Text to be inserted
%
% ### Examples
%
% ```latex
% \begin{table}[t]
%     \centering
%     \begin{tabular}{llr}
%         \hline
%         \multicolumn{2}{c}{Item} \\
%         \cline{1-2}
%         Animal                  & Description & Price (\$)          \\
%         \hline
%         \multirow{2}{*}{Gnat*}  & per gram                  & 13.65 \\
%                                 & each                      & 0.01  \\
%         Gnu                     & \multirow{2}{*}{stuffed*} & 92.50 \\
%         Emu                     &                           & 33.33 \\
%         Armadillo & frozen      & 8.99                              \\
%         \hline
%     \end{tabular}
%     \caption{A table.}
%     \label{tab:table}
% \end{table}
% ```
%
% CTAN: https://ctan.org/pkg/multirow

\usepackage{multirow}

% ## Use natbib – Flexible bibliography support
%
% This package provides options to manage bibliography items.
%
% ### Usage
%
% #### Citation Commands
%
% This package provides two citation commands:
% ```latex
% \citet[<post-note>]{<ref>}
% \citep[<pre-note>][<post-note>]{<ref>}
% \citet*[<post-note>]{<ref>}
% \citep*[<pre-note>][<post-note>]{<ref>}
% ```
% `citet` is for textual citations and `citep` is for parenthetical citations. The starred versions print the full author list.
%
% #### Bibliography Styles
%
% You also have to set the bibliography style by `\bibliographystyle{<style>}`:
% 1. "plainnat": natbib version of the standard plain (numerical only) style
% 2. "abbrvnat": natbib version of the standard abbrv (abbreviated author names) style
% 3. "unsrtnat": natbib version of the standard unsrt (references are listed in order of citation) style
%
% #### Citation Punctuation
%
% You can customize citation punctuation by `\setcitestyle{<style>}`:
% 1. Citation mode:
%   1. "authoryear": Author-year (default)
%   2. "numbers": Numerical
%   3. "super": Superscripts for numerical citations
% 2. Braces:
%   1. "round": Round (default)
%   2. "square": Square
% 3. Between citations:
%   1. "semicolon": Semicolon
%   2. "comma": Comma (default)
% 4. Between author and year: `aysep={<char>}` (Default: `;`)
% 5. Between years with common author: `yysep={<char>}` (Default: `,`)
% 6. Text before `<post-note>`: `notesep={<text>}` (Default: `, `)
%
% For more advanced usage, please see the documentation on CTAN.
%
% ### Examples
%
% #### Citation Commands
%
% 1. `\citet{jon90}`: Jones et al. (1990)
% 2. `\citep{jon90}`: (Jones et al., 1990)
% 3. `\citet[chap. 2]{jon90}`: Jones et al. (1990, chap. 2)
% 4. `\citep[see][chap. 2]{jon90}`: (see Jones et al., 1990, chap. 2)
% 5. `\citet*{jon90}`: Jones, Baker, and Williams (1990)
% 6. `\citep*{jon90}`: (Jones, Baker, and Williams, 1990)
% 7. `\citet{jon90,jam91}`: Jones et al. (1990); James et al. (1991)
% 8. `\citep{jon90,jam91}`: (Jones et al., 1990; James et al. 1991)
%
% #### Bibliography Styles
%
% ```latex
% \bibliographystyle{plainnat}
% \bibliographystyle{abbrvnat}
% \bibliographystyle{unsrtnat}
% ```
%
% #### Citation Punctuation
%
% The defaults of the citation punctuation style is set by:
% ```latex
% \setcitestyle{authoryear,round,comma,aysep={;},yysep={,},notesep={, }}
% ```
%
% CTAN: https://ctan.org/pkg/natbib
% References:
% 1. http://merkel.texture.rocks/Latex/natbib.php
% 2. https://www.overleaf.com/learn/latex/Bibliography_management_with_natbib
% 3. https://www.overleaf.com/learn/latex/Bibtex%20bibliography%20styles

% \usepackage{natbib}

% ## Use setspace – Set space between lines
%
% This package allows you to adjust the spacing between lines in a document.
%
% ### Usage
%
% Use the environment `\begin{spacing}{<stretch>}` to surround the content to be stretched. Smaller `<stretch>` will have less vertical spacing. Default `<stretch>` is `1`.
%
% ### Examples
%
% Reduce the vertical spacing between equations:
% ```latex
% \begin{spacing}{0.5}
%     \begin{equation}
%         x=y
%     \end{equation}
%     \begin{equation}
%         x=y
%     \end{equation}
% \end{spacing}
% ```
%
% CTAN: https://ctan.org/pkg/setspace
% Reference: https://texblog.org/2011/09/30/quick-note-on-line-spacing/

\usepackage{setspace}

% ## Use subcaption – Support for sub-captions
%
% This package allows you to creates subfigures and corresponding captions.
%
% This package is not compatible with the "subfig" package.
%
% ### Usage
%
% Use environment `subfigure` for subfigures and `subtable` for subtables. Use command `\subcaption` to add sub-captions. You can add more horizontal spacing between each subfloat by either `~`, `\quad`, `\qquad` or `\hfill`, or add a blank line to force the subfloat onto a new line. You can use `\captionsetup{skip=<spacing>}` inside the `subfigure` or `subtable` environment to raise up the content.
%
% ### Examples
%
% To have 3 subfigures, add:
% ```latex
% \begin{figure}[t]
%     \centering
%     \begin{subfigure}[b]{0.3\linewidth}
%         \includegraphics[width=\textwidth]{gull.png}
%         \subcaption{A gull.}
%         \label{fig:gull}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.3\linewidth}
%         \includegraphics[width=\textwidth]{tiger.png}
%         \subcaption{A tiger.}
%         \label{fig:tiger}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.3\linewidth}
%         \includegraphics[width=\textwidth]{mouse.png}
%         \subcaption{A mouse.}
%         \label{fig:mouse}
%     \end{subfigure}
%     \caption{Pictures of animals.}
%     \label{fig:animals}
% \end{figure}
% ```
%
% To have 3 subtables, add:
% ```latex
% \begin{table}[t]
%     \centering
%     \begin{subtable}[b]{0.3\linewidth}
%         \centering
%         \begin{tabular}{lcr}
%             \hline
%             1 & 2 & 3 \\
%             \hline
%             4 & 5 & 6 \\
%             7 & 8 & 9 \\
%             \hline
%         \end{tabular}
%         \subcaption{Subtable 1.}
%         \label{tab:subtable1}
%     \end{subtable}
%     \begin{subtable}[b]{0.3\linewidth}
%         \centering
%         \begin{tabular}{lcr}
%             \hline
%             1 & 2 & 3 \\
%             \hline
%             4 & 5 & 6 \\
%             7 & 8 & 9 \\
%             \hline
%         \end{tabular}
%         \subcaption{Subtable 2.}
%         \label{tab:subtable2}
%     \end{subtable}
%     \begin{subtable}[b]{0.3\linewidth}
%         \centering
%         \begin{tabular}{lcr}
%             \hline
%             1 & 2 & 3 \\
%             \hline
%             4 & 5 & 6 \\
%             7 & 8 & 9 \\
%             \hline
%         \end{tabular}
%         \subcaption{Subtable 3.}
%         \label{tab:subtable3}
%     \end{subtable}
%     \caption{Some sub-tables.}
%     \label{tab:subtables}
% \end{table}
% ```
%
% You can also mix subfigures and subtables together by replacing either `subfigure` or `subtable` environment with one another, and replace the content accordingly.
%
% CTAN: https://ctan.org/pkg/subcaption
% Reference: https://en.wikibooks.org/wiki/LaTeX/Floats,_Figures_and_Captions

%\usepackage{subcaption}

% ## Use subfig – Figures broken into subfigures
%
% This package allows you to creates subfigures and corresponding captions.
%
% This package is not compatible with the "subcaption" package. It's the alternative of the package "subcaption" when there are compatibility issues with it.
%
% ### Usage
%
% Use the command `\subfloat[<sub-caption>]{<body>}` to create subfigures and subtables. You can add more horizontal spacing between each subfloat by either `~`, `\quad`, `\qquad` or `\hfill`, or add a blank line to force the subfloat onto a new line. You can add a `\raisebox{<spacing>}{<captionsetup-and-subfloat-command>}` and add a `\captionsetup[subfloat]{captionskip=<spacing>}` inside `<captionsetup-and-subfloat-command>` to raise up `<body>` and align the subcaption with side-by-side subcaptions.
%
% ### Examples
%
% To have 3 subfigures, add:
% ```latex
% \begin{figure}[t]
%     \centering
%     \subfloat[A gull.\label{fig:gull}]{\includegraphics[width=0.3\linewidth]{gull.png}}
%     \subfloat[A tiger.\label{fig:tiger}]{\includegraphics[width=0.3\linewidth]{tiger.png}}
%     \subfloat[A mouse.\label{fig:mouse}]{\includegraphics[width=0.3\linewidth]{mouse.png}}
%     \caption{Pictures of animals.}
%     \label{fig:animals}
% \end{figure}
% ```
%
% To have 3 subtables, add:
% ```latex
% \begin{table}[t]
%     \centering
%     \subfloat[Subtable 1.\label{tab:subtable1}]{
%         \begin{tabular}{lcr}
%             \hline
%             1 & 2 & 3 \\
%             \hline
%             4 & 5 & 6 \\
%             7 & 8 & 9 \\
%             \hline
%         \end{tabular}
%     }
%     \subfloat[Subtable 2.\label{tab:subtable2}]{
%         \begin{tabular}{lcr}
%             \hline
%             1 & 2 & 3 \\
%             \hline
%             4 & 5 & 6 \\
%             7 & 8 & 9 \\
%             \hline
%         \end{tabular}
%     }
%     \subfloat[Subtable 3.\label{tab:subtable3}]{
%         \begin{tabular}{lcr}
%             \hline
%             1 & 2 & 3 \\
%             \hline
%             4 & 5 & 6 \\
%             7 & 8 & 9 \\
%             \hline
%         \end{tabular}
%     }
%     \caption{Some sub-tables.}
%     \label{tab:subtables}
% \end{table}
% ```
%
% You can also mix subfigures and subtables together by replacing the `<body>` with either subfigure or subtable.
%
% CTAN: https://ctan.org/pkg/subfig

\usepackage{subfig}

% ## Use tabu – Flexible LATEX tabulars
%
% This package provides more flexibility to adjust widths of tables.
%
% ### Usage
%
% Available environment options are:
% 1. `\begin{tabu}{<preamble>}`: Behave like "tabular", the widths of columns are determined automatically
% 2. `\begin{tabu} to <dimen> {<preamble>}`: Behave like "tabular*", the table will be stretched to the width of `<dimen>`
% 3. `\begin{tabu} spread <dimen> {<preamble>}`: Make the table wider than the width of `<dimen>`
% You should use the column specified `X[<width-coeff>]` or `X[<width-coeff>,<horizontal-align>]`.
% `<width-coeff>` is the width coefficient. It is an integer specifying the relative width to the other columns. For example, the column with `X[2.5]` will be two and half wider than the column with `X[1]`
% `horizontal-align` is the horizontal alignment specification. Available options are:
% 1. `l` or `L`: Left-justified column
% 2. `c` or `C`: Center-justified column
% 3. `r` or `R`: Right-justified column
% 4. `j` or `J`: Normal-justified column (Default)
%
% For more advanced usage, please see the documentation on CTAN.
%
% ### Examples
%
% ```latex
% \begin{table}[t]
%     \centering
%     \begin{tabu} to 0.9\linewidth {|X[2,l]|X[1,c]|X[2,r]|X[2]|}
%         \hline
%         label 1     & label 2   & label 3     & label 4     \\
%         \hline
%         long item 1 & item 2    & long item 3 & long item 4 \\
%         \hline
%     \end{tabu}
%     \caption{A table.}
%     \label{tab:table}
% \end{table}
% ```
%
% CTAN: https://ctan.org/pkg/tabu
% Reference: https://en.wikibooks.org/wiki/LaTeX/Tables

\usepackage{tabu}

% ## Use tabularx – Tabulars with adjustable-width columns
%
% This package provides more flexibility to adjust widths of tables.
%
% ### Usage
%
% Use the environment `\begin{tabularx}{<width>}{<preamble>}`. Available options are:
% 1. `width`: Desired width of table.
% 2. `preamble`: You can add the column specifier `X` to have the columns stretched to make the table as wide as specified by `width`
%
% ### Examples
%
% You can add the following column types to have different alignments:
% ```latex
% % Left-aligned
% \newcolumntype{L}{>{\raggedright\arraybackslash}X}
% % Right-aligned
% \newcolumntype{R}{>{\raggedleft\arraybackslash}X}
% % Center-aligned
% \newcolumntype{C}{>{\centering\arraybackslash}X}
% ```
% For example:
% ```latex
% \begin{table}[t]
%     \centering
%     \begin{tabularx}{0.9\linewidth}{|L|C|R|X|}
%         \hline
%         label 1     & label 2   & label 3     & label 4     \\
%         \hline
%         long item 1 & item 2    & long item 3 & long item 4 \\
%         \hline
%     \end{tabularx}
%     \caption{A table.}
%     \label{tab:table}
% \end{table}
% ```
%
% CTAN: https://ctan.org/pkg/tabularx
% Reference: https://en.wikibooks.org/wiki/LaTeX/Tables

\usepackage{tabularx}

% ## Use tabulary – Tabular with variable width columns balanced
%
% This package provides more flexibility to adjust widths of tables.
%
% This package tries to balance the column widths so that each column has at least its natural width, without exceeding the maximum length. The problem with "tabularx" is that it leaves much blank if your cells are almost empty.
%
% ### Usage
%
% Use the environment `\begin{tabulary}{<length>}{<pream>}`. Available options are:
% 1. `length`: Desired width of table.
% 2. `pream`: You can add following column specifiers:
%   1. `L`: Left-justified balanced column
%   2. `C`: Center-justified balanced column
%   3. `R`: Right-justified balanced column
%   4. `J`: Normally-justified balanced column
%
% ### Examples
%
% ```latex
% \begin{table}[t]
%     \centering
%     \begin{tabulary}{0.9\linewidth}{|L|C|R|J|}
%         \hline
%         label 1     & label 2   & label 3     & label 4     \\
%         \hline
%         long item 1 & item 2    & long item 3 & long item 4 \\
%         \hline
%     \end{tabulary}
%     \caption{A table.}
%     \label{tab:table}
% \end{table}
% ```
%
% CTAN: https://ctan.org/pkg/tabulary
% Reference: https://en.wikibooks.org/wiki/LaTeX/Tables

\usepackage{tabulary}

% ## Use titlesec – Select alternative section titles
%
% This package is used for adjusting spacing before and after section titles.
%
% ### Usage
%
% To adjust the vertical spacing before and after the section titles, write:
% ```latex
% \titlespacing{<command>}{<left>}{<before-sep>}{<after-sep>}
% ```
% Available options are:
% 1. `command`: Command to be adjusted
% 2. `left`: Horizontal spacing on the left side of the command
% 3. `before-sep`: Vertical spacing before the command
% 4. `after-sep`: Vertical spacing after the command
%
% For more advanced usage, please see the documentation on CTAN.
%
% ### Examples
%
% To have specific spacing, set the values directly:
% ```latex
% \titlespacing{\section}{0pt}{3.5ex plus 1ex minus .2ex}{2.3ex plus .2ex}
% ```
%
% To have relative spacing to default spacing, set the multiplication:
% ```latex
% \titlespacing{\section}{0pt}{*.5}{*.5}
% ```
%
% CTAN: https://ctan.org/pkg/titlesec

\usepackage{titlesec}

% ## Use xfrac – Split-level fractions in LATEX2ε*
%
% This package allows the user to typeset fractions in the form ‘n/d’.
%
% ### Usage
%
% To insert fraction in the form "n/d", write:
% ```latex
% \sfrac{<num>}{<denom>}
% ```
%
% ### Examples
%
% To insert the fraction "1/2", write:
% ```latex
% $\sfrac{1}{2}$
% ```
%
% CTAN: https://ctan.org/pkg/xfrac

\usepackage{xfrac}

\usepackage[
]{algorithmic}


==> Model-based Lookahead Reinforcement Learning (NIPS2019) (3)/custom2.tex <==
% # Customization 2
%
% This file determines the features to use controlled by variable "draftmode", or apply other features to use regardless of "draftmode". The features here should override other configurations.

% You can safely comment the following packages and customization if not used.

\ifbool{draftmode}{
    %%% Draft mode is on %%%

    % ## Draft Mode Reminder
    %
    % Set the color to magenta to remind the editor to turn off draft mode before submitting.

    \newcommand{\draftmodereminder}{\color{magenta}}

    % ## Use hyperref – Extensive support for hypertext in LATEX
    %
    % This package allows you to write commands to produce hypertext links.
    %
    % ### Usage
    %
    % Some common commands include:
    % ```latex
    % \href{<URL>}{<text>}
    % \url{<URL>}
    % \hyperref[<label>]{<text>}
    % ```
    %
    % ### Examples
    %
    % Add the following line in document:
    % ```latex
    % \href{https://google.com}{Google}
    % \url{https://google.com}
    % Section~\hyperref[sec:intro]{\ref*{sec:intro}}
    % ```
    %
    % ### Options
    %
    % 1. `pagebackref=true` adds ‘backlink’ text to the end of each item in the bibliography, as a list of page numbers
    % 2. `bookmarks=false` turns off Acrobat bookmarks
    %
    % CTAN: https://ctan.org/pkg/hyperref
    % Reference: https://en.wikibooks.org/wiki/LaTeX/Hyperlinks

    \usepackage[
        pagebackref=true,
        bookmarks=false
    ]{hyperref}

    % ## Customize fixme
    %
    % Show FiXme annotations inline and with color.

    \ifdef{\fxsetup}{
        \fxsetup{
            status=draft,
            layout=inline,
            author=,
            theme=color
        }
    }{
    }

    % ## Customize hyperref
    %
    % Make hyperlinks easy to be spotted.

    \ifdef{\hypersetup}{
        \hypersetup{
            % Colors the text of links and anchors
            colorlinks=true,
            % Color for normal internal links
            linkcolor=blue,
            % Color for bibliographical citations in text
            citecolor=red,
            % Color for linked URLs
            urlcolor=blue
        }
    }{
    }
}{
    %%% Draft mode is off %%%

    % ## Draft Mode Reminder
    %
    % Set the command to empty to clear the color.

    \newcommand{\draftmodereminder}{}

    % ## Use hyperref – Extensive support for hypertext in LATEX
    %
    % This package allows you to write commands to produce hypertext links.
    %
    % ### Usage
    %
    % Some common commands include:
    % ```latex
    % \href{<URL>}{<text>}
    % \url{<URL>}
    % \hyperref[<label>]{<text>}
    % ```
    %
    % ### Examples
    %
    % Add the following line in document:
    % ```latex
    % \href{https://google.com}{Google}
    % \url{https://google.com}
    % Section~\hyperref[sec:intro]{\ref*{sec:intro}}
    % ```
    %
    % ### Options
    %
    % 1. `bookmarks=false` turns off Acrobat bookmarks
    %
    % CTAN: https://ctan.org/pkg/hyperref
    % Reference: https://en.wikibooks.org/wiki/LaTeX/Hyperlinks

    \usepackage[
        bookmarks=false
    ]{hyperref}

    % ## Customize fixme
    %
    % Hide FiXme annotations.

    \ifdef{\fxsetup}{
        \fxsetup{
            status=final
        }
    }{
    }
}

%%% Regardless of draft mode %%%

% ## Customize Fixed-length Spaces
%
% Change vertical spacing of the commands `\smallskip`, `\medskip` and `\largeskip`.
% It is not recommended to adjust these spacing. It is wiser to reduce words.

% Vertical spacing of `\smallskip`
% \setlength{\smallskipamount}{3.0pt plus 1.0pt minus 1.0pt}
% Vertical spacing of `\medskip`
% \setlength{\medskipamount}{6.0pt plus 2.0pt minus 2.0pt}
% Vertical spacing of `\largeskip`
% \setlength{\bigskipamount}{12.0pt plus 4.0pt minus 4.0pt}

% ## Customize Layout
%
% Change vertical spacing between floats and texts.
% It is not recommended to adjust these spacing. It is wiser to use smaller figures or reduce words.

% Vertical spacing between two floats
\setlength{\floatsep}{0.5ex}
% Vertical spacing between last float and first text line
\setlength{\textfloatsep}{0.5ex}
% % Vertical spacing between two floats (in two-column mode)
% \setlength{\dblfloatsep}{2ex}
% % Vertical spacing between last float and first text line (in two-column mode)
% \setlength{\dbltextfloatsep}{1ex}

% ## Customize Paragraph Formatting
%
% Change paragraph spacing.
% It is not recommended to adjust the paragraph spacing. It is wiser to reduce words.
%
% Reference: https://en.wikibooks.org/wiki/LaTeX/Paragraph_Formatting

% Horizontal spacing before the first line of a paragraph
% \setlength{\parindent}{1em}
% Vertical spacing between two paragraphs
\setlength{\parskip}{5pt plus 1pt}

% ## Use algorithm2e – Floating algorithm environment with algorithmic keywords
%
% This package provides a floating environment for wrapping pseudocode and provides commands for writing pseudocode.
%
% This package is not compatible with the following packages:
% 1. algorithm
% 2. algorithmic
% 3. algpseudocode
%
% ### Package Options (Section 7)
%
% Add one of the following options or omit to use default behavior in each subsection.
%
% #### Environment Display (Section 7.3.1)
%
% 1. `ruled`: Have algorithms with a line at the top and the bottom
% 2. `plain`: Print algorithms without any surrounding lines (Default)
%
% #### Blocks Display (Section 7.4.2)
%
% 1. `lined`: Print vertical lines between start and end keywords (Default)
% 2. `noline`: Do not print vertical lines between start and end keywords
%
% #### End Keywords (Section 7.4.3)
%
% 1. `shortend`: Print "end" for end keywords (Default)
% 2. `noend`: Do not print any end keywords
%
% #### Line Numbers (Section 7.4.5)
%
% 1. `linesnumbered`: Show line numbers
% 2. `linesnumberedhidden`: Hide line numbers (Default)
%
% ### Commands (Section 9)
%
% Put the following commands in the beginning of the "algorithm" environment:
% 1. `\DontPrintSemicolon`: Do not print semicolons at the end of each line
% 2. `\BlankLine`: Print a blank line
% 3. `\SetAlgoCaptionSeparator{<sep>}`: Set the separator between title of algorithms and the name of the algorithm
% 4. `\SetKwSty{<font>}`: Set the Kw typography (e.g., `if`) (Default: `textbf`)
% 5. `\SetProgSty{<font>}`: Set the KwProg typography (e.g., conditions in `if`) (Default: `emph`)
%
% ### Usage
%
% End each simple statement with `\;`.
%
% This package provides the following commands.
%
% #### Input and Output (Section 10.1)
%
% ```latex
% \KwIn{<input>}
% \KwOut{<output>}
% \KwData{<input>}
% \KwResult{<output>}
% ```
%
% #### Basic Keywords and Blocks (Section 10.2)
%
% ```latex
% \KwTo
% \KwRet{<value>}
% \Begin{<block>}
% ```
%
% #### if-then-else (Section 10.4)
%
% ```latex
% \If{<condition>}{<block>}
% \ElseIf{<block>}
% \Else{<block>}
% ```
%
% #### Multiple Condition Selection (Section 10.5)
%
% ```latex
% \Switch{<condition>}{<block>}
% \Case{<case>}{<block>}
% \Other{<block>}
% ```
%
% #### Loop with End Condition At the Beginning
%
% ```latex
% \For{<condition>}{<loop>}
% \While{<condition>}{<loop>}
% \ForEach{<condition>}{<loop>}
% \ForAll{<condition>}{<loop>}
% ```
%
% #### Loop with End Condition At the End
%
% ```latex
% \Repeat{<condition>}{<loop>}
% ```
%
% For more advanced usage, please see the documentation on CTAN.
%
% ### Examples
%
% The following example reproduces the algorithm in the paper "Playing Atari with Deep Reinforcement Learning":
% ```latex
% \begin{algorithm*}[t]
%     % Do not print semicolons
%     \DontPrintSemicolon
%     % Remove caption separator
%     \SetAlgoCaptionSeparator{}
%     % Use default font for programm type
%     \SetProgSty{textnormal}

%     \caption{Deep Q-learning with Experience Replay}
%     \label{alg:algorithm}
%     Initialize replay memory $\mathcal{D}$ to capacity $N$\;
%     Initialize action-value function $Q$ with random weights\;
%     \For{episode $=1,M$}{
%         Initialize sequence $s_1=\{x_1\}$ and preprocessed sequenced $\phi_1=\phi(s_1)$\;
%         \For{$t=1,T$}{
%             With probability $\epsilon$ select a random action $a_t$\;
%             otherwise select $a_t=\max_a Q*(\phi(s_t),a;\theta)$\;
%             Execute action $a_t$ in emulator and observe reward $r_t$ and image $x_{t+1}$\;
%             Set $s_{t+1}=s_t,a_t,x_{t+1}$ and preprocess $\phi_{t+1}=\phi(s_{t+1})$\;
%             Store transition $(\phi_t,a_t,r_t,\phi_{t+1})$ in $\mathcal{D}$\;
%             Sample random minibatch of transitions $(\phi_j,a_j,r_j,\phi_{j+1})$ from $\mathcal{D}$\;
%             Set $y_j=
%                 \begin{cases}
%                     r_j & \text{for terminal } \phi_{j+1} \\
%                     r_j+\gamma\max_{a'}Q(\phi_{j+1},a';\theta) & \text{for non-terminal } \phi_{j+1}
%                 \end{cases}$\;
%             Perform a gradient descent step on $(y_j-Q(\phi_j,a_j;\theta))^2$ according to equation 3\;\label{op:gradient}
%         }
%     }
% \end{algorithm*}
% ```
%
% CTAN: https://ctan.org/pkg/algorithm2e
% Reference: https://en.wikibooks.org/wiki/LaTeX/Algorithms

% \usepackage[
%     ruled,
%     noline,
%     linesnumbered
% ]{algorithm2e}

% ## Use algorithmic
%
% This package provides commands for writing pseudocode.
%
% This package is not compatible with the following packages:
% 1. algorithmicx
% 2. algpseudocode
% 3. algorithm2e
%
% ### Package Options
%
% Add the option `noend` to omit "end" statements.
%
% ### Usage
%
% This package provides the following commands.
%
% #### Simple Statement (Section 3.1)
%
% ```latex
% \STATE <text>
% ```
%
% #### if-then-else (Section 3.2)
%
% ```latex
% \IF{<condition>} <text> \ENDIF
% \IF{<condition>} <text1> \ELSE <text2> \ENDIF
% \IF{<condition1>} <text1> \ELSIF{<condition2>} <text2> \ELSE <text3> \ENDIF
% ```
%
% #### for Loop (Section 3.3)
%
% ```latex
% \FOR{<condition>} <text> \ENDFOR
% \FORALL{<condition>} <text> \ENDFOR
% ```
%
% #### while Loop (Section 3.4)
%
% ```latex
% \WHILE{<condition>} <text> \ENDWHILE
% ```
%
% #### repeat-until Loop (Section 3.5)
%
% ```latex
% \REPEAT <text> \UNTIL{<condition>}
% ```
%
% #### Infinite Loop (Section 3.6)
%
% ```latex
% \LOOP <text> \ENDLOOP
% ```
%
% #### Logical Connectives (Section 3.7)
%
% ```latex
% <expression> \AND <expression>
% <expression> \OR <expression>
% <expression> \XOR <expression>
% \NOT <expression>
% ```
%
% #### Precondition (Section 3.8)
%
% ```latex
% \REQUIRE <text>
% ```
%
% #### Postcondition (Section 3.9)
%
% ```latex
% \ENSURE <text>
% ```
%
% #### Returning Values (Section 3.10)
%
% ```latex
% \RETURN <text>
% ```
%
% #### Comments (Section 3.12)
%
% ```latex
% \COMMENT{<text>}
% ```
%
% #### Other Commands
%
% 1. You can use `\TO` inside `<condition>` to specify ranges (Section 3.3.1):
%   ```latex
%   <expression> \TO <expression>
%   ```
% 2. You can use `\TRUE` and `\FALSE` to specify boolean values (Section 3.10.1):
%   ```latex
%   <expression> \TRUE
%   <expression> \FALSE
%   ```
%
% #### Labels and References
%
% Insert `\label{<label>}` at the end of a line and use `\ref{<label>}` to add a reference to the line number.
%
% ### Examples
%
% The following example reproduces the algorithm in the paper "Playing Atari with Deep Reinforcement Learning":
% ```latex
% \begin{algorithm*}[t]
%     \caption{Deep Q-learning with Experience Replay}
%     \label{alg:algorithm}
%     \begin{algorithmic}
%         \STATE Initialize replay memory $\mathcal{D}$ to capacity $N$
%         \STATE Initialize action-value function $Q$ with random weights
%         \FOR{episode $=1,M$}
%             \STATE Initialize sequence $s_1=\{x_1\}$ and preprocessed sequenced $\phi_1=\phi(s_1)$
%             \FOR{$t=1,T$}
%                 \STATE With probability $\epsilon$ select a random action $a_t$
%                 \STATE otherwise select $a_t=\max_a Q*(\phi(s_t),a;\theta)$
%                 \STATE Execute action $a_t$ in emulator and observe reward $r_t$ and image $x_{t+1}$
%                 \STATE Set $s_{t+1}=s_t,a_t,x_{t+1}$ and preprocess $\phi_{t+1}=\phi(s_{t+1})$
%                 \STATE Store transition $(\phi_t,a_t,r_t,\phi_{t+1})$ in $\mathcal{D}$
%                 \STATE Sample random minibatch of transitions $(\phi_j,a_j,r_j,\phi_{j+1})$ from $\mathcal{D}$
%                 \STATE Set $y_j=
%                     \begin{cases}
%                         r_j & \text{for terminal } \phi_{j+1} \\
%                         r_j+\gamma\max_{a'}Q(\phi_{j+1},a';\theta) & \text{for non-terminal } \phi_{j+1}
%                     \end{cases}$
%                 \STATE Peform a gradient descent step on $(y_j-Q(\phi_j,a_j;\theta))^2$ according to equation 3 \label{op:gradient}
%             \ENDFOR
%         \ENDFOR
%     \end{algorithmic}
% \end{algorithm*}
% ```
% Note: The above example requires the "algorithm" package.
%
% CTAN: https://ctan.org/pkg/algorithms
% Reference: https://en.wikibooks.org/wiki/LaTeX/Algorithms

\usepackage[
]{algorithmic}

% ## Use algpseudocode
%
% This package is a layout for "algorithmicx" package.
%
% It provides predefined commands to be used with the "algorithmicx" package together. This layout has almost the same look as the one in "algorithmic" package. Since this package loads the "algorithmicx" package internally, there is no need to require the "algorithmicx" package.
%
% This package is not compatible with the following packages:
% 1. algorithmic
% 2. algorithm2e
%
% ### Package Options
%
% Add the option `noend` to omit "end" statements.
%
% ### Usage
%
% This package provides the following commands.
%
% #### Simple Lines (Section 2.3)
%
% ```latex
% \State <body>
% ```
%
% #### for Block (Section 3.1.1)
%
% ```latex
% \For{<text>}
%   <body>
% \EndFor
%
% \ForAll{<text>}
%   <body>
% \EndFor
% ```
%
% #### while Block (Section 3.1.2)
%
% ```latex
% \While{<text>}
%   <body>
% \EndWhile
% ```
%
% #### repeat Block (Section 3.1.3)
%
% ```latex
% \Repeat
%   <body>
% \Until{<text>}
% ```
%
% #### if Block (Section 3.1.4)
%
% ```latex
% \If{<text>}
%   <body>
% \EndIf
%
% \If{<text>}
%   <body>
% \Else
%   <body>
% \EndIf
%
% \If{<text>}
%   <body>
% \ElsIf{<text>}
%   <body>
% \Else
%   <body>
% \EndIf
% ```
%
% #### procedure Block (Section 3.1.5)
%
% ```latex
% \Procedure{<name>}{<params>}
%   <body>
% \EndProcedure
% ```
%
% #### function Block (Section 3.1.6)
%
% ```latex
% \Function{<name>}{<params>}
%   <body>
% \EndFunction
% ```
%
% #### loop Block (Section 3.1.7)
%
% ```latex
% \Loop
%   <body>
% \EndLoop
% ```
%
% #### Other Commands (Section 3.1.8)
%
% 1. Add precondition:
%   ```latex
%   \Require <body>
%   ```
% 2. Add postcondition:
%   ```latex
%   \Ensure <body>
%   ```
% 3. Add a blank line:
%   ```latex
%   \Statex
%   ```
% 4. Add a procedure call:
%   ```latex
%   \State \Call{<name>}{<params>}
%   ```
% 5. Add a return statement:
%   ```latex
%   \State \Return
%   ```
%
% #### Custom Commands
%
% If you want a easy solution to define commands, simply use `\textbf{<command>}`, for example:
% ```latex
% \For{$i=1$ \textbf{to} $N$}
%     \State \textbf{print} $i$
% \EndFor
% \State \Return \textbf{true}
% ```
%
% #### Labels and References
%
% Insert `\label{<label>}` at the end of a line and use `\ref{<label>}` to add a reference to the line number.
%
% ### Examples
%
% The following example reproduces the algorithm in the paper "Playing Atari with Deep Reinforcement Learning":
% ```latex
% \begin{algorithm*}[t]
%     \caption{Deep Q-learning with Experience Replay}
%     \label{alg:algorithm}
%     \begin{algorithmic}
%         \State Initialize replay memory $\mathcal{D}$ to capacity $N$
%         \State Initialize action-value function $Q$ with random weights
%         \For{episode $=1,M$}
%             \State Initialize sequence $s_1=\{x_1\}$ and preprocessed sequenced $\phi_1=\phi(s_1)$
%             \For{$t=1,T$}
%                 \State With probability $\epsilon$ select a random action $a_t$
%                 \State otherwise select $a_t=\max_a Q*(\phi(s_t),a;\theta)$
%                 \State Execute action $a_t$ in emulator and observe reward $r_t$ and image $x_{t+1}$
%                 \State Set $s_{t+1}=s_t,a_t,x_{t+1}$ and preprocess $\phi_{t+1}=\phi(s_{t+1})$
%                 \State Store transition $(\phi_t,a_t,r_t,\phi_{t+1})$ in $\mathcal{D}$
%                 \State Sample random minibatch of transitions $(\phi_j,a_j,r_j,\phi_{j+1})$ from $\mathcal{D}$
%                 \State Set $y_j=
%                     \begin{cases}
%                         r_j & \text{for terminal } \phi_{j+1} \\
%                         r_j+\gamma\max_{a'}Q(\phi_{j+1},a';\theta) & \text{for non-terminal } \phi_{j+1}
%                     \end{cases}$
%                 \State Peform a gradient descent step on $(y_j-Q(\phi_j,a_j;\theta))^2$ according to equation 3 \label{op:gradient}
%             \EndFor
%         \EndFor
%     \end{algorithmic}
% \end{algorithm*}
% ```
% Note: The above example requires the "algorithm" package.
%
% CTAN: https://ctan.org/pkg/algorithmicx
% Reference: https://en.wikibooks.org/wiki/LaTeX/Algorithms

% \usepackage[
% ]{algpseudocode}

% ## Use BibLATEX – Sophisticated Bibliographies in LATEX
%
% This package provides options to manage bibliography items.
%
% ### Usage
%
% 1. Replace `\bibliographystyle` and `\bibliography` with a single line `\printbibliography`
%
% ### Load-time Options (Section 3.1.1)
%
% The following options must be set in optional arguments to `\usepackage`:
% 1. `style`: Set both the bibliography and citation styles (Default: `numeric`)
% 2. `bibstyle`: Set the bibliography style only (Default: `numeric`)
% 3. `citestyle`: Set the citation style only (Default: `numeric`)
% 4. `natbib`: Provide aliases for the citation commands of the "natbib" package
% Rather than setting both `bibstyle` and `citestyle`, setting `style` is usually enough.
%
% ### Preamble Options (Section 3.1.2)
%
% The following options can be either set in optional arguments to `\usepackage` or by the command `\ExecuteBibliographyOptions{<key=value, ...>}`:
% 1. `sorting=<value>`: The sorting order of the bibliography. The entries are sorted in ascending order. Available values are:
%   1. `nty`: Sort by name, title, year (default)
%   2. `nyt`: Sort by name, year, title
%   3. `nyvt`: Sort by name, year, volume, title
%   4. `anyt`: Sort by alphabetic label, name, year, title
%   5. `anyvt`: Sort by alphabetic label, name, year, volume, title
%   6. `ynt`: Sort by year, name, title
%   7. `ydnt`: Sort by year (descending), name, title
%   8. `none`: Do not sort at all. All entries are processed in citation order
% 2. `sortcites=<bool>`: Whether or not to sort citations if multiple entry keys are passed to a citation command (Default: `false`)
% 3. `maxnames=<int>`: If a list holds more than `<int>` names, it is truncated according to the `minnames` option (Default: `3`)
% 4. `minnames=<int>`: If a list holds more than `maxnames` names, it is truncated to `minnames` names (Default: `1`)
% 5. `autocite=<value>`: Control translation of `\autocite` command. Available values are:
%   1. `plain`: Make `\autocite` behave like `\cite`
%   2. `inline`: Make `\autocite` behave like `\parencite`
%   3. `footnote`: Make `\autocite` behave like `\footcite`
%   4. `superscript`: Make `\autocite` behave like `\supercite` (Only in `numeric` citation style)
%   The default setting depends on the selected citation style.
% 6. `autopunct=<bool>`: Control whether the citation commands scan ahead for punctuation mark to avoid spurious punctuation marks after citations (Default: `true`)
% 7. `block=<value>`: Control the extra spacing between blocks. Available values are:
%   1. `none`: Do not add anything at all
%   2. `space`: Insert additional horizontal space between blocks
%   3. `par`: Start a new paragraph for every block
%   4. `nbpar`: Similar to the `par` option, but disallows page breaks at block boundaries and within an entry
%   5. `ragged`: Insert a small negative penalty to encourage line breaks at block boundaries and set the bibliography ragged right
% 8. `backref=<bool>`: Whether or not to print back references in the bibliography (Default: `false`)
%   Note: If you want to turn on this feature, remember to turn off `pagebackref` option in "hyperref" package because they are not compatible
% 9. `date=<value>`: Controls the basic format of printed date specifications. Available values are:
%   1. `year`: Use only years (e.g., "2010", "2010-2012")
%   2. `short`: Use the short format with verbose ranges (e.g., "01/01/2010", "01/21/2010–01/30/2010")
%   3. `long`: Use the long format with verbose ranges (e.g., "1st January 2010", "January 21, 2010–January 30, 2010")
%   4. `terse`: Use the short format with compact ranges (e.g., "01/21–01/30/2010")
%   5. `comp`: Use the long format with compact ranges (e.g., "January 21–30, 2010") (default)
%   6. `iso`: Use ISO8601 Extended Format (yyyy-mm-dd) (e.g., "2010-01-01", "2010-01-21/2010-01-30")
%   If you want to customize more, search "datetype" in the CTAN documentation.
% 10. `datezeros=<bool>`: Control whether `short` and `terse` date components are printed with leading zeros (Default: `true`)
% 11. `dateabbrev=<bool>`: Control whether long and comp dates are printed with long or abbreviated month/season names (Default: `true`)
%
% ### Citation Styles (Section 3.3.1)
%
% 1. `numeric`: Numeric citation scheme (e.g., "[1]")
% 2. `alphabetic`: Alphabetic citation scheme (e.g., "[Mni+13]")
% 3. `authoryear`: Author-year citation scheme (e.g., "Mnih et al. 2013")
% 4. `authortitle`: Author-title citation scheme (e.g., "Mnih et al., “Playing atari with deep reinforcement learn-ing”")
% 5. `verbose`: Verbose citation scheme (e.g., "Volodymyr Mnih et al. “Playing atari with deep reinforcement learn-ing”. In:arXiv preprint arXiv:1312.5602(2013).")
% 6. `reading`: The citation is the same as `authortitle`
% 7. `draft`: Use entry keys in citations (e.g., "mnih2013playing")
%
% ### Bibliography Styles (Section 3.3.2)
%
% 1. `numeric`: Print numeric labels (e.g., "[1]")
% 2. `alphabetic`: Print alphabetic labels (e.g., "[Mni+13]")
% 3. `authoryear`: Print Author-year label before other entries (e.g., "Mnih et al. (2013)")
% 4. `authortitle`: Does not print any label
% 5. `verbose`: Does not print any label
% 6. `reading`: Print personal reading lists
% 7. `draft`: Print entry keys. The bibliography will be sorted by entry key (e.g., "mnih2013playing")
%
% ### Citation Commands (Section 3.8)
%
% 1. `\cite[<prenote>][<postnote>]{<key>}`: Print the citation without any  parentheses
% 2. `\parencite[<prenote>][<postnote>]{<key>}`: Enclose the entire citation in parentheses (Counterpart of `\citep` in "natbib" package)
% 3. `\footcite[<prenote>][<postnote>]{<key>}`: Put the entire citation in a footnote and add a period at the end
% 4. `\textcite[<prenote>][<postnote>]{<key>}`: Print the authors or editors followed by a citation label which is enclosed in parentheses (Counterpart of `\citet` in "natbib" package)
% 5. `\supercite[<prenote>][<postnote>]{<key>}`: Print numeric citations as superscripts without brackets
% 6. `\autocite[<prenote>][<postnote>]{<key>}`: Translate into the lower-level citation command most appropriate for the style family (controlled by `autocite` option)
%
% For more advanced usage, please see the documentation on CTAN.
%
% CTAN: https://ctan.org/pkg/biblatex
% References:
% 1. https://www.overleaf.com/learn/latex/Articles/Getting_started_with_BibLaTeX
% 2. https://www.overleaf.com/learn/latex/Bibliography_management_in_LaTeX
% 3. https://www.overleaf.com/learn/latex/Biblatex_bibliography_styles
% 4. https://www.overleaf.com/learn/latex/Biblatex_citation_styles
% 5. https://tex.stackexchange.com/a/58592
% 6. https://tex.stackexchange.com/a/5095

% \usepackage[
% ]{biblatex}

% ## Use cite – Improved citation handling in LATEX
%
% This package provides options to manage bibliography items.
%
% ### Options
%
% The default settings is to turn on every feature, add the following options to to disable them:
% 1. `nospace`: Eliminate the spaces after commas in the number list (e.g., [1,2,3])
% 2. `nosort`: Prevent sorting of the numbers
% 3. `nomove`: Prevent moving the superscript cite after punctuation
% 4. `noadjust`: Disable ‘smart’ handling of space before a cite
% 5. `nocompress`: Inhibit compression of consecutive numbers into ranges
%
% CTAN: https://ctan.org/pkg/cite

% \usepackage[
% ]{cite}

% ## Customize biblatex
%
% 1. Import bibtex data file
% 2. Set preamble options

\ifdef{\addbibresource}{
    % Replace `references.bib` with proper file
    \addbibresource{references.bib}
    % Set preamble options
    \ExecuteBibliographyOptions{
    }
}{
}

% ## Customize booktabs
%
% 1. Change line widths
% 2. Change vertical spacing before and after lines

\ifdef{\heavyrulewidth}{
    % Change line width for `\toprule` and `\bottomrule`
    \setlength{\heavyrulewidth}{.08em}
    % Change line width for `\midrule`
    \setlength{\lightrulewidth}{.05em}
    % Change line width for `cmidrule`
    \setlength{\cmidrulewidth}{.03em}
    % Change vertical spacing before lines except `\toprule`
    \setlength{\aboverulesep}{0ex}
    % Change vertical spacing after lines except `\bottomrule`
    \setlength{\belowrulesep}{0ex}
    % Change vertical spacing between two `\cmidrule`
    \setlength{\cmidrulesep}{\doublerulesep}
}{
}

% ## Customize caption
%
% 1. Change font sizes
% 2. Change vertical spacing after figures, tables, and subfigures.
% In the case that these settings fail to change the desired spacing, it is recommended to use commands like `\smallskip`, `\medskip` or `\bigskip` if there is not enough spacing.
% It is not recommended to adjust these spacing. It is wiser to use smaller tables or reduce words.

\ifdef{\captionsetup}{
    % Customize figure environment
    \captionsetup[figure]{
        % Font size option
        font=small,
        % Vertical space between float and caption
        skip=1ex
    }
    % Customize table environment
    \captionsetup[table]{
        % Font size options
        font=small,
        % Vertical space between float and caption
        skip=1ex
    }
    % Customize subcaption environment
    \ifdef{\subcaption}{
        % \captionsetup[sub]{
        %     % Font size options
        %     font=small,
        %     % Vertical space between sub-float and sub-caption
        %     skip=1ex
        % }
    }{
    }
    % Customize subfig environment
    \ifdef{\subfloat}{
        \captionsetup[subfloat]{
            % Font size option
            font=small,
            % Vertical space between sub-float and sub-caption
            captionskip=1ex,
            % Vertical space between float and caption
            nearskip=1ex
        }
    }{
    }
}{
}

% ## Customize enumitem
%
% Change vertical spacing between items.

\ifdef{\setlist}{
    \setlist{
        % Vertical spacing before and after the item area
        topsep=0ex,
        % Vertical spacing before and after the item area if there are blank lines
        partopsep=0ex,
        % Vertical spacing between two paragraphs
        parsep=0ex,
        % Vertical spacing between two items
        itemsep=0.5ex
    }
}{
}

% ## Customize geometry
%
% Change ratio of body text to paper size.
% It is not recommended to adjust these spacing. It is wiser to reduce words.

\ifdef{\geometry}{
    % \geometry{
    %     % Ratio of width of total body to paper width
    %     hscale=0.75,
    %     % Ratio of height of total body to paper height
    %     vscale=0.75
    % }
}{
}

% ## Customize natbib
%
% Change citation punctuation.

\ifdef{\setcitestyle}{
    \setcitestyle{
    }
}{
}

% ## Customize tabu
%
% Change vertical spacing between the cell content and the cell border.

\ifcsdef{tabu}{
    % Set the minimal vertical space allowed between the cell content and the cell border
    \setlength{\tabulinesep}{2pt}
}{
}

% ## Customize titlesec
%
% Change vertical spacing before and after section titles.
% It is not recommended to adjust these spacing. It is wiser to reduce words.

\ifdef{\titlespacing}{
    % section
    \titlespacing{\section}{0pt}{*0}{*0}
    % subsection
    \titlespacing{\subsection}{0pt}{*0}{*0}
    % subsubsection
    \titlespacing{\subsubsection}{0pt}{*0}{*0}
    % paragraph
    \titlespacing{\paragraph}{0pt}{*0}{*0}
    % subparagraph
    \titlespacing{\subparagraph}{0pt}{*0}{*0}
}{
}


==> custom2.tex <==
% # Customization 2
%
% This file determines the features to use controlled by variable "draftmode", or apply other features to use regardless of "draftmode". The features here should override other configurations.

% You can safely comment the following packages and customization if not used.

\ifbool{draftmode}{
    %%% Draft mode is on %%%

    % ## Draft Mode Reminder
    %
    % Set the color to magenta to remind the editor to turn off draft mode before submitting.

    \newcommand{\draftmodereminder}{\color{magenta}}

    % ## Use hyperref – Extensive support for hypertext in LATEX
    %
    % This package allows you to write commands to produce hypertext links.
    %
    % ### Usage
    %
    % Some common commands include:
    % ```latex
    % \href{<URL>}{<text>}
    % \url{<URL>}
    % \hyperref[<label>]{<text>}
    % ```
    %
    % ### Examples
    %
    % Add the following line in document:
    % ```latex
    % \href{https://google.com}{Google}
    % \url{https://google.com}
    % Section~\hyperref[sec:intro]{\ref*{sec:intro}}
    % ```
    %
    % ### Options
    %
    % 1. `pagebackref=true` adds ‘backlink’ text to the end of each item in the bibliography, as a list of page numbers
    % 2. `bookmarks=false` turns off Acrobat bookmarks
    %
    % CTAN: https://ctan.org/pkg/hyperref
    % Reference: https://en.wikibooks.org/wiki/LaTeX/Hyperlinks

    \usepackage[
        pagebackref=true,
        bookmarks=false
    ]{hyperref}

    % ## Customize fixme
    %
    % Show FiXme annotations inline and with color.

    \ifdef{\fxsetup}{
        \fxsetup{
            status=draft,
            layout=inline,
            author=,
            theme=color
        }
    }{
    }

    % ## Customize hyperref
    %
    % Make hyperlinks easy to be spotted.

    \ifdef{\hypersetup}{
        \hypersetup{
            % Colors the text of links and anchors
            colorlinks=true,
            % Color for normal internal links
            linkcolor=blue,
            % Color for bibliographical citations in text
            citecolor=red,
            % Color for linked URLs
            urlcolor=blue
        }
    }{
    }
}{
    %%% Draft mode is off %%%

    % ## Draft Mode Reminder
    %
    % Set the command to empty to clear the color.

    \newcommand{\draftmodereminder}{}

    % ## Use hyperref – Extensive support for hypertext in LATEX
    %
    % This package allows you to write commands to produce hypertext links.
    %
    % ### Usage
    %
    % Some common commands include:
    % ```latex
    % \href{<URL>}{<text>}
    % \url{<URL>}
    % \hyperref[<label>]{<text>}
    % ```
    %
    % ### Examples
    %
    % Add the following line in document:
    % ```latex
    % \href{https://google.com}{Google}
    % \url{https://google.com}
    % Section~\hyperref[sec:intro]{\ref*{sec:intro}}
    % ```
    %
    % ### Options
    %
    % 1. `bookmarks=false` turns off Acrobat bookmarks
    %
    % CTAN: https://ctan.org/pkg/hyperref
    % Reference: https://en.wikibooks.org/wiki/LaTeX/Hyperlinks

    \usepackage[
        bookmarks=false
    ]{hyperref}

    % ## Customize fixme
    %
    % Hide FiXme annotations.

    \ifdef{\fxsetup}{
        \fxsetup{
            status=final
        }
    }{
    }
}

%%% Regardless of draft mode %%%

% ## Customize Fixed-length Spaces
%
% Change vertical spacing of the commands `\smallskip`, `\medskip` and `\largeskip`.
% It is not recommended to adjust these spacing. It is wiser to reduce words.

% Vertical spacing of `\smallskip`
% \setlength{\smallskipamount}{3.0pt plus 1.0pt minus 1.0pt}
% Vertical spacing of `\medskip`
% \setlength{\medskipamount}{6.0pt plus 2.0pt minus 2.0pt}
% Vertical spacing of `\largeskip`
% \setlength{\bigskipamount}{12.0pt plus 4.0pt minus 4.0pt}

% ## Customize Layout
%
% Change vertical spacing between floats and texts.
% It is not recommended to adjust these spacing. It is wiser to use smaller figures or reduce words.

% Vertical spacing between two floats
\setlength{\floatsep}{0.5ex}
% Vertical spacing between last float and first text line
\setlength{\textfloatsep}{0.5ex}
% % Vertical spacing between two floats (in two-column mode)
% \setlength{\dblfloatsep}{2ex}
% % Vertical spacing between last float and first text line (in two-column mode)
% \setlength{\dbltextfloatsep}{1ex}

% ## Customize Paragraph Formatting
%
% Change paragraph spacing.
% It is not recommended to adjust the paragraph spacing. It is wiser to reduce words.
%
% Reference: https://en.wikibooks.org/wiki/LaTeX/Paragraph_Formatting

% Horizontal spacing before the first line of a paragraph
% \setlength{\parindent}{1em}
% Vertical spacing between two paragraphs
\setlength{\parskip}{5pt plus 1pt}

% ## Use algorithm2e – Floating algorithm environment with algorithmic keywords
%
% This package provides a floating environment for wrapping pseudocode and provides commands for writing pseudocode.
%
% This package is not compatible with the following packages:
% 1. algorithm
% 2. algorithmic
% 3. algpseudocode
%
% ### Package Options (Section 7)
%
% Add one of the following options or omit to use default behavior in each subsection.
%
% #### Environment Display (Section 7.3.1)
%
% 1. `ruled`: Have algorithms with a line at the top and the bottom
% 2. `plain`: Print algorithms without any surrounding lines (Default)
%
% #### Blocks Display (Section 7.4.2)
%
% 1. `lined`: Print vertical lines between start and end keywords (Default)
% 2. `noline`: Do not print vertical lines between start and end keywords
%
% #### End Keywords (Section 7.4.3)
%
% 1. `shortend`: Print "end" for end keywords (Default)
% 2. `noend`: Do not print any end keywords
%
% #### Line Numbers (Section 7.4.5)
%
% 1. `linesnumbered`: Show line numbers
% 2. `linesnumberedhidden`: Hide line numbers (Default)
%
% ### Commands (Section 9)
%
% Put the following commands in the beginning of the "algorithm" environment:
% 1. `\DontPrintSemicolon`: Do not print semicolons at the end of each line
% 2. `\BlankLine`: Print a blank line
% 3. `\SetAlgoCaptionSeparator{<sep>}`: Set the separator between title of algorithms and the name of the algorithm
% 4. `\SetKwSty{<font>}`: Set the Kw typography (e.g., `if`) (Default: `textbf`)
% 5. `\SetProgSty{<font>}`: Set the KwProg typography (e.g., conditions in `if`) (Default: `emph`)
%
% ### Usage
%
% End each simple statement with `\;`.
%
% This package provides the following commands.
%
% #### Input and Output (Section 10.1)
%
% ```latex
% \KwIn{<input>}
% \KwOut{<output>}
% \KwData{<input>}
% \KwResult{<output>}
% ```
%
% #### Basic Keywords and Blocks (Section 10.2)
%
% ```latex
% \KwTo
% \KwRet{<value>}
% \Begin{<block>}
% ```
%
% #### if-then-else (Section 10.4)
%
% ```latex
% \If{<condition>}{<block>}
% \ElseIf{<block>}
% \Else{<block>}
% ```
%
% #### Multiple Condition Selection (Section 10.5)
%
% ```latex
% \Switch{<condition>}{<block>}
% \Case{<case>}{<block>}
% \Other{<block>}
% ```
%
% #### Loop with End Condition At the Beginning
%
% ```latex
% \For{<condition>}{<loop>}
% \While{<condition>}{<loop>}
% \ForEach{<condition>}{<loop>}
% \ForAll{<condition>}{<loop>}
% ```
%
% #### Loop with End Condition At the End
%
% ```latex
% \Repeat{<condition>}{<loop>}
% ```
%
% For more advanced usage, please see the documentation on CTAN.
%
% ### Examples
%
% The following example reproduces the algorithm in the paper "Playing Atari with Deep Reinforcement Learning":
% ```latex
% \begin{algorithm*}[t]
%     % Do not print semicolons
%     \DontPrintSemicolon
%     % Remove caption separator
%     \SetAlgoCaptionSeparator{}
%     % Use default font for programm type
%     \SetProgSty{textnormal}

%     \caption{Deep Q-learning with Experience Replay}
%     \label{alg:algorithm}
%     Initialize replay memory $\mathcal{D}$ to capacity $N$\;
%     Initialize action-value function $Q$ with random weights\;
%     \For{episode $=1,M$}{
%         Initialize sequence $s_1=\{x_1\}$ and preprocessed sequenced $\phi_1=\phi(s_1)$\;
%         \For{$t=1,T$}{
%             With probability $\epsilon$ select a random action $a_t$\;
%             otherwise select $a_t=\max_a Q*(\phi(s_t),a;\theta)$\;
%             Execute action $a_t$ in emulator and observe reward $r_t$ and image $x_{t+1}$\;
%             Set $s_{t+1}=s_t,a_t,x_{t+1}$ and preprocess $\phi_{t+1}=\phi(s_{t+1})$\;
%             Store transition $(\phi_t,a_t,r_t,\phi_{t+1})$ in $\mathcal{D}$\;
%             Sample random minibatch of transitions $(\phi_j,a_j,r_j,\phi_{j+1})$ from $\mathcal{D}$\;
%             Set $y_j=
%                 \begin{cases}
%                     r_j & \text{for terminal } \phi_{j+1} \\
%                     r_j+\gamma\max_{a'}Q(\phi_{j+1},a';\theta) & \text{for non-terminal } \phi_{j+1}
%                 \end{cases}$\;
%             Perform a gradient descent step on $(y_j-Q(\phi_j,a_j;\theta))^2$ according to equation 3\;\label{op:gradient}
%         }
%     }
% \end{algorithm*}
% ```
%
% CTAN: https://ctan.org/pkg/algorithm2e
% Reference: https://en.wikibooks.org/wiki/LaTeX/Algorithms

% \usepackage[
%     ruled,
%     noline,
%     linesnumbered
% ]{algorithm2e}

% ## Use algorithmic
%
% This package provides commands for writing pseudocode.
%
% This package is not compatible with the following packages:
% 1. algorithmicx
% 2. algpseudocode
% 3. algorithm2e
%
% ### Package Options
%
% Add the option `noend` to omit "end" statements.
%
% ### Usage
%
% This package provides the following commands.
%
% #### Simple Statement (Section 3.1)
%
% ```latex
% \STATE <text>
% ```
%
% #### if-then-else (Section 3.2)
%
% ```latex
% \IF{<condition>} <text> \ENDIF
% \IF{<condition>} <text1> \ELSE <text2> \ENDIF
% \IF{<condition1>} <text1> \ELSIF{<condition2>} <text2> \ELSE <text3> \ENDIF
% ```
%
% #### for Loop (Section 3.3)
%
% ```latex
% \FOR{<condition>} <text> \ENDFOR
% \FORALL{<condition>} <text> \ENDFOR
% ```
%
% #### while Loop (Section 3.4)
%
% ```latex
% \WHILE{<condition>} <text> \ENDWHILE
% ```
%
% #### repeat-until Loop (Section 3.5)
%
% ```latex
% \REPEAT <text> \UNTIL{<condition>}
% ```
%
% #### Infinite Loop (Section 3.6)
%
% ```latex
% \LOOP <text> \ENDLOOP
% ```
%
% #### Logical Connectives (Section 3.7)
%
% ```latex
% <expression> \AND <expression>
% <expression> \OR <expression>
% <expression> \XOR <expression>
% \NOT <expression>
% ```
%
% #### Precondition (Section 3.8)
%
% ```latex
% \REQUIRE <text>
% ```
%
% #### Postcondition (Section 3.9)
%
% ```latex
% \ENSURE <text>
% ```
%
% #### Returning Values (Section 3.10)
%
% ```latex
% \RETURN <text>
% ```
%
% #### Comments (Section 3.12)
%
% ```latex
% \COMMENT{<text>}
% ```
%
% #### Other Commands
%
% 1. You can use `\TO` inside `<condition>` to specify ranges (Section 3.3.1):
%   ```latex
%   <expression> \TO <expression>
%   ```
% 2. You can use `\TRUE` and `\FALSE` to specify boolean values (Section 3.10.1):
%   ```latex
%   <expression> \TRUE
%   <expression> \FALSE
%   ```
%
% #### Labels and References
%
% Insert `\label{<label>}` at the end of a line and use `\ref{<label>}` to add a reference to the line number.
%
% ### Examples
%
% The following example reproduces the algorithm in the paper "Playing Atari with Deep Reinforcement Learning":
% ```latex
% \begin{algorithm*}[t]
%     \caption{Deep Q-learning with Experience Replay}
%     \label{alg:algorithm}
%     \begin{algorithmic}
%         \STATE Initialize replay memory $\mathcal{D}$ to capacity $N$
%         \STATE Initialize action-value function $Q$ with random weights
%         \FOR{episode $=1,M$}
%             \STATE Initialize sequence $s_1=\{x_1\}$ and preprocessed sequenced $\phi_1=\phi(s_1)$
%             \FOR{$t=1,T$}
%                 \STATE With probability $\epsilon$ select a random action $a_t$
%                 \STATE otherwise select $a_t=\max_a Q*(\phi(s_t),a;\theta)$
%                 \STATE Execute action $a_t$ in emulator and observe reward $r_t$ and image $x_{t+1}$
%                 \STATE Set $s_{t+1}=s_t,a_t,x_{t+1}$ and preprocess $\phi_{t+1}=\phi(s_{t+1})$
%                 \STATE Store transition $(\phi_t,a_t,r_t,\phi_{t+1})$ in $\mathcal{D}$
%                 \STATE Sample random minibatch of transitions $(\phi_j,a_j,r_j,\phi_{j+1})$ from $\mathcal{D}$
%                 \STATE Set $y_j=
%                     \begin{cases}
%                         r_j & \text{for terminal } \phi_{j+1} \\
%                         r_j+\gamma\max_{a'}Q(\phi_{j+1},a';\theta) & \text{for non-terminal } \phi_{j+1}
%                     \end{cases}$
%                 \STATE Peform a gradient descent step on $(y_j-Q(\phi_j,a_j;\theta))^2$ according to equation 3 \label{op:gradient}
%             \ENDFOR
%         \ENDFOR
%     \end{algorithmic}
% \end{algorithm*}
% ```
% Note: The above example requires the "algorithm" package.
%
% CTAN: https://ctan.org/pkg/algorithms
% Reference: https://en.wikibooks.org/wiki/LaTeX/Algorithms

\usepackage[
]{algorithmic}

% ## Use algpseudocode
%
% This package is a layout for "algorithmicx" package.
%
% It provides predefined commands to be used with the "algorithmicx" package together. This layout has almost the same look as the one in "algorithmic" package. Since this package loads the "algorithmicx" package internally, there is no need to require the "algorithmicx" package.
%
% This package is not compatible with the following packages:
% 1. algorithmic
% 2. algorithm2e
%
% ### Package Options
%
% Add the option `noend` to omit "end" statements.
%
% ### Usage
%
% This package provides the following commands.
%
% #### Simple Lines (Section 2.3)
%
% ```latex
% \State <body>
% ```
%
% #### for Block (Section 3.1.1)
%
% ```latex
% \For{<text>}
%   <body>
% \EndFor
%
% \ForAll{<text>}
%   <body>
% \EndFor
% ```
%
% #### while Block (Section 3.1.2)
%
% ```latex
% \While{<text>}
%   <body>
% \EndWhile
% ```
%
% #### repeat Block (Section 3.1.3)
%
% ```latex
% \Repeat
%   <body>
% \Until{<text>}
% ```
%
% #### if Block (Section 3.1.4)
%
% ```latex
% \If{<text>}
%   <body>
% \EndIf
%
% \If{<text>}
%   <body>
% \Else
%   <body>
% \EndIf
%
% \If{<text>}
%   <body>
% \ElsIf{<text>}
%   <body>
% \Else
%   <body>
% \EndIf
% ```
%
% #### procedure Block (Section 3.1.5)
%
% ```latex
% \Procedure{<name>}{<params>}
%   <body>
% \EndProcedure
% ```
%
% #### function Block (Section 3.1.6)
%
% ```latex
% \Function{<name>}{<params>}
%   <body>
% \EndFunction
% ```
%
% #### loop Block (Section 3.1.7)
%
% ```latex
% \Loop
%   <body>
% \EndLoop
% ```
%
% #### Other Commands (Section 3.1.8)
%
% 1. Add precondition:
%   ```latex
%   \Require <body>
%   ```
% 2. Add postcondition:
%   ```latex
%   \Ensure <body>
%   ```
% 3. Add a blank line:
%   ```latex
%   \Statex
%   ```
% 4. Add a procedure call:
%   ```latex
%   \State \Call{<name>}{<params>}
%   ```
% 5. Add a return statement:
%   ```latex
%   \State \Return
%   ```
%
% #### Custom Commands
%
% If you want a easy solution to define commands, simply use `\textbf{<command>}`, for example:
% ```latex
% \For{$i=1$ \textbf{to} $N$}
%     \State \textbf{print} $i$
% \EndFor
% \State \Return \textbf{true}
% ```
%
% #### Labels and References
%
% Insert `\label{<label>}` at the end of a line and use `\ref{<label>}` to add a reference to the line number.
%
% ### Examples
%
% The following example reproduces the algorithm in the paper "Playing Atari with Deep Reinforcement Learning":
% ```latex
% \begin{algorithm*}[t]
%     \caption{Deep Q-learning with Experience Replay}
%     \label{alg:algorithm}
%     \begin{algorithmic}
%         \State Initialize replay memory $\mathcal{D}$ to capacity $N$
%         \State Initialize action-value function $Q$ with random weights
%         \For{episode $=1,M$}
%             \State Initialize sequence $s_1=\{x_1\}$ and preprocessed sequenced $\phi_1=\phi(s_1)$
%             \For{$t=1,T$}
%                 \State With probability $\epsilon$ select a random action $a_t$
%                 \State otherwise select $a_t=\max_a Q*(\phi(s_t),a;\theta)$
%                 \State Execute action $a_t$ in emulator and observe reward $r_t$ and image $x_{t+1}$
%                 \State Set $s_{t+1}=s_t,a_t,x_{t+1}$ and preprocess $\phi_{t+1}=\phi(s_{t+1})$
%                 \State Store transition $(\phi_t,a_t,r_t,\phi_{t+1})$ in $\mathcal{D}$
%                 \State Sample random minibatch of transitions $(\phi_j,a_j,r_j,\phi_{j+1})$ from $\mathcal{D}$
%                 \State Set $y_j=
%                     \begin{cases}
%                         r_j & \text{for terminal } \phi_{j+1} \\
%                         r_j+\gamma\max_{a'}Q(\phi_{j+1},a';\theta) & \text{for non-terminal } \phi_{j+1}
%                     \end{cases}$
%                 \State Peform a gradient descent step on $(y_j-Q(\phi_j,a_j;\theta))^2$ according to equation 3 \label{op:gradient}
%             \EndFor
%         \EndFor
%     \end{algorithmic}
% \end{algorithm*}
% ```
% Note: The above example requires the "algorithm" package.
%
% CTAN: https://ctan.org/pkg/algorithmicx
% Reference: https://en.wikibooks.org/wiki/LaTeX/Algorithms

% \usepackage[
% ]{algpseudocode}

% ## Use BibLATEX – Sophisticated Bibliographies in LATEX
%
% This package provides options to manage bibliography items.
%
% ### Usage
%
% 1. Replace `\bibliographystyle` and `\bibliography` with a single line `\printbibliography`
%
% ### Load-time Options (Section 3.1.1)
%
% The following options must be set in optional arguments to `\usepackage`:
% 1. `style`: Set both the bibliography and citation styles (Default: `numeric`)
% 2. `bibstyle`: Set the bibliography style only (Default: `numeric`)
% 3. `citestyle`: Set the citation style only (Default: `numeric`)
% 4. `natbib`: Provide aliases for the citation commands of the "natbib" package
% Rather than setting both `bibstyle` and `citestyle`, setting `style` is usually enough.
%
% ### Preamble Options (Section 3.1.2)
%
% The following options can be either set in optional arguments to `\usepackage` or by the command `\ExecuteBibliographyOptions{<key=value, ...>}`:
% 1. `sorting=<value>`: The sorting order of the bibliography. The entries are sorted in ascending order. Available values are:
%   1. `nty`: Sort by name, title, year (default)
%   2. `nyt`: Sort by name, year, title
%   3. `nyvt`: Sort by name, year, volume, title
%   4. `anyt`: Sort by alphabetic label, name, year, title
%   5. `anyvt`: Sort by alphabetic label, name, year, volume, title
%   6. `ynt`: Sort by year, name, title
%   7. `ydnt`: Sort by year (descending), name, title
%   8. `none`: Do not sort at all. All entries are processed in citation order
% 2. `sortcites=<bool>`: Whether or not to sort citations if multiple entry keys are passed to a citation command (Default: `false`)
% 3. `maxnames=<int>`: If a list holds more than `<int>` names, it is truncated according to the `minnames` option (Default: `3`)
% 4. `minnames=<int>`: If a list holds more than `maxnames` names, it is truncated to `minnames` names (Default: `1`)
% 5. `autocite=<value>`: Control translation of `\autocite` command. Available values are:
%   1. `plain`: Make `\autocite` behave like `\cite`
%   2. `inline`: Make `\autocite` behave like `\parencite`
%   3. `footnote`: Make `\autocite` behave like `\footcite`
%   4. `superscript`: Make `\autocite` behave like `\supercite` (Only in `numeric` citation style)
%   The default setting depends on the selected citation style.
% 6. `autopunct=<bool>`: Control whether the citation commands scan ahead for punctuation mark to avoid spurious punctuation marks after citations (Default: `true`)
% 7. `block=<value>`: Control the extra spacing between blocks. Available values are:
%   1. `none`: Do not add anything at all
%   2. `space`: Insert additional horizontal space between blocks
%   3. `par`: Start a new paragraph for every block
%   4. `nbpar`: Similar to the `par` option, but disallows page breaks at block boundaries and within an entry
%   5. `ragged`: Insert a small negative penalty to encourage line breaks at block boundaries and set the bibliography ragged right
% 8. `backref=<bool>`: Whether or not to print back references in the bibliography (Default: `false`)
%   Note: If you want to turn on this feature, remember to turn off `pagebackref` option in "hyperref" package because they are not compatible
% 9. `date=<value>`: Controls the basic format of printed date specifications. Available values are:
%   1. `year`: Use only years (e.g., "2010", "2010-2012")
%   2. `short`: Use the short format with verbose ranges (e.g., "01/01/2010", "01/21/2010–01/30/2010")
%   3. `long`: Use the long format with verbose ranges (e.g., "1st January 2010", "January 21, 2010–January 30, 2010")
%   4. `terse`: Use the short format with compact ranges (e.g., "01/21–01/30/2010")
%   5. `comp`: Use the long format with compact ranges (e.g., "January 21–30, 2010") (default)
%   6. `iso`: Use ISO8601 Extended Format (yyyy-mm-dd) (e.g., "2010-01-01", "2010-01-21/2010-01-30")
%   If you want to customize more, search "datetype" in the CTAN documentation.
% 10. `datezeros=<bool>`: Control whether `short` and `terse` date components are printed with leading zeros (Default: `true`)
% 11. `dateabbrev=<bool>`: Control whether long and comp dates are printed with long or abbreviated month/season names (Default: `true`)
%
% ### Citation Styles (Section 3.3.1)
%
% 1. `numeric`: Numeric citation scheme (e.g., "[1]")
% 2. `alphabetic`: Alphabetic citation scheme (e.g., "[Mni+13]")
% 3. `authoryear`: Author-year citation scheme (e.g., "Mnih et al. 2013")
% 4. `authortitle`: Author-title citation scheme (e.g., "Mnih et al., “Playing atari with deep reinforcement learn-ing”")
% 5. `verbose`: Verbose citation scheme (e.g., "Volodymyr Mnih et al. “Playing atari with deep reinforcement learn-ing”. In:arXiv preprint arXiv:1312.5602(2013).")
% 6. `reading`: The citation is the same as `authortitle`
% 7. `draft`: Use entry keys in citations (e.g., "mnih2013playing")
%
% ### Bibliography Styles (Section 3.3.2)
%
% 1. `numeric`: Print numeric labels (e.g., "[1]")
% 2. `alphabetic`: Print alphabetic labels (e.g., "[Mni+13]")
% 3. `authoryear`: Print Author-year label before other entries (e.g., "Mnih et al. (2013)")
% 4. `authortitle`: Does not print any label
% 5. `verbose`: Does not print any label
% 6. `reading`: Print personal reading lists
% 7. `draft`: Print entry keys. The bibliography will be sorted by entry key (e.g., "mnih2013playing")
%
% ### Citation Commands (Section 3.8)
%
% 1. `\cite[<prenote>][<postnote>]{<key>}`: Print the citation without any  parentheses
% 2. `\parencite[<prenote>][<postnote>]{<key>}`: Enclose the entire citation in parentheses (Counterpart of `\citep` in "natbib" package)
% 3. `\footcite[<prenote>][<postnote>]{<key>}`: Put the entire citation in a footnote and add a period at the end
% 4. `\textcite[<prenote>][<postnote>]{<key>}`: Print the authors or editors followed by a citation label which is enclosed in parentheses (Counterpart of `\citet` in "natbib" package)
% 5. `\supercite[<prenote>][<postnote>]{<key>}`: Print numeric citations as superscripts without brackets
% 6. `\autocite[<prenote>][<postnote>]{<key>}`: Translate into the lower-level citation command most appropriate for the style family (controlled by `autocite` option)
%
% For more advanced usage, please see the documentation on CTAN.
%
% CTAN: https://ctan.org/pkg/biblatex
% References:
% 1. https://www.overleaf.com/learn/latex/Articles/Getting_started_with_BibLaTeX
% 2. https://www.overleaf.com/learn/latex/Bibliography_management_in_LaTeX
% 3. https://www.overleaf.com/learn/latex/Biblatex_bibliography_styles
% 4. https://www.overleaf.com/learn/latex/Biblatex_citation_styles
% 5. https://tex.stackexchange.com/a/58592
% 6. https://tex.stackexchange.com/a/5095

% \usepackage[
% ]{biblatex}

% ## Use cite – Improved citation handling in LATEX
%
% This package provides options to manage bibliography items.
%
% ### Options
%
% The default settings is to turn on every feature, add the following options to to disable them:
% 1. `nospace`: Eliminate the spaces after commas in the number list (e.g., [1,2,3])
% 2. `nosort`: Prevent sorting of the numbers
% 3. `nomove`: Prevent moving the superscript cite after punctuation
% 4. `noadjust`: Disable ‘smart’ handling of space before a cite
% 5. `nocompress`: Inhibit compression of consecutive numbers into ranges
%
% CTAN: https://ctan.org/pkg/cite

% \usepackage[
% ]{cite}

% ## Customize biblatex
%
% 1. Import bibtex data file
% 2. Set preamble options

\ifdef{\addbibresource}{
    % Replace `references.bib` with proper file
    \addbibresource{references.bib}
    % Set preamble options
    \ExecuteBibliographyOptions{
    }
}{
}

% ## Customize booktabs
%
% 1. Change line widths
% 2. Change vertical spacing before and after lines

\ifdef{\heavyrulewidth}{
    % Change line width for `\toprule` and `\bottomrule`
    \setlength{\heavyrulewidth}{.08em}
    % Change line width for `\midrule`
    \setlength{\lightrulewidth}{.05em}
    % Change line width for `cmidrule`
    \setlength{\cmidrulewidth}{.03em}
    % Change vertical spacing before lines except `\toprule`
    \setlength{\aboverulesep}{0ex}
    % Change vertical spacing after lines except `\bottomrule`
    \setlength{\belowrulesep}{0ex}
    % Change vertical spacing between two `\cmidrule`
    \setlength{\cmidrulesep}{\doublerulesep}
}{
}

% ## Customize caption
%
% 1. Change font sizes
% 2. Change vertical spacing after figures, tables, and subfigures.
% In the case that these settings fail to change the desired spacing, it is recommended to use commands like `\smallskip`, `\medskip` or `\bigskip` if there is not enough spacing.
% It is not recommended to adjust these spacing. It is wiser to use smaller tables or reduce words.

\ifdef{\captionsetup}{
    % Customize figure environment
    \captionsetup[figure]{
        % Font size option
        font=small,
        % Vertical space between float and caption
        skip=1ex
    }
    % Customize table environment
    \captionsetup[table]{
        % Font size options
        font=small,
        % Vertical space between float and caption
        skip=1ex
    }
    % Customize subcaption environment
    \ifdef{\subcaption}{
        % \captionsetup[sub]{
        %     % Font size options
        %     font=small,
        %     % Vertical space between sub-float and sub-caption
        %     skip=1ex
        % }
    }{
    }
    % Customize subfig environment
    \ifdef{\subfloat}{
        \captionsetup[subfloat]{
            % Font size option
            font=small,
            % Vertical space between sub-float and sub-caption
            captionskip=1ex,
            % Vertical space between float and caption
            nearskip=1ex
        }
    }{
    }
}{
}

% ## Customize enumitem
%
% Change vertical spacing between items.

\ifdef{\setlist}{
    \setlist{
        % Vertical spacing before and after the item area
        topsep=0ex,
        % Vertical spacing before and after the item area if there are blank lines
        partopsep=0ex,
        % Vertical spacing between two paragraphs
        parsep=0ex,
        % Vertical spacing between two items
        itemsep=0.5ex
    }
}{
}

% ## Customize geometry
%
% Change ratio of body text to paper size.
% It is not recommended to adjust these spacing. It is wiser to reduce words.

\ifdef{\geometry}{
    % \geometry{
    %     % Ratio of width of total body to paper width
    %     hscale=0.75,
    %     % Ratio of height of total body to paper height
    %     vscale=0.75
    % }
}{
}

% ## Customize natbib
%
% Change citation punctuation.

\ifdef{\setcitestyle}{
    \setcitestyle{
    }
}{
}

% ## Customize tabu
%
% Change vertical spacing between the cell content and the cell border.

\ifcsdef{tabu}{
    % Set the minimal vertical space allowed between the cell content and the cell border
    \setlength{\tabulinesep}{2pt}
}{
}

% ## Customize titlesec
%
% Change vertical spacing before and after section titles.
% It is not recommended to adjust these spacing. It is wiser to reduce words.

\ifdef{\titlespacing}{
    % section
    \titlespacing{\section}{0pt}{*0}{*0}
    % subsection
    \titlespacing{\subsection}{0pt}{*0}{*0}
    % subsubsection
    \titlespacing{\subsubsection}{0pt}{*0}{*0}
    % paragraph
    \titlespacing{\paragraph}{0pt}{*0}{*0}
    % subparagraph
    \titlespacing{\subparagraph}{0pt}{*0}{*0}
}{
}

